Numerical investigations of the fluid-structure interaction of a NACA0012 airfoil based on large-eddy simulations

The purpose of this work is to expand the work of Streher (2017) in order to investigate the aeroelastic instabilities generated by the flow around a moving NACA0012 airfoil. The profile has a chord length of $c=0.1 m and is exposed to a flow at a Reynolds number of Re=30,000. The airfoil has only two degrees of freedom: Translation in relation to the vertical direction and a rotation around the span-wise axis. A partitioned approach based on two separate solvers and a fluid-structure interaction (FSI) coupling scheme is applied. The in-house CFD solver FASTEST-3D computes the fluid sub-problem according to the wall-resolved large-eddy simulation (LES) combined with the Smagorinsky model (1963). The structural sub-problem is solved by a rigid movement solver implemented by Viets (2013), which is based on the equations of motion for rigid bodies. The FSI coupling exchanges information between both solvers based on loose or strong coupling algorithms. A thorough analysis of the problem is primarily performed in order to acquire a computational setup that provides the best compromise between accuracy and CPU-time requirements. Three system configurations are then tested and thoroughly investigated: One leads to an oscillatory behavior of the airfoil characterized by limited small amplitudes. The other is characterized by the presence of the torsional divergence aeroelastic instability. Finally, a configuration aimed at the flutter phenomenon is established. However, not enough data are currently available and therefore this dynamic aeroelastic instability can not be thoroughly investigated in the present work. In the near future, this study will serve as a base for the flutter experiments and computations performed at the Department of Fluid Mechanics located of the Helmut-Schmidt-University.

==> 2.tex <==
\chapter{Preliminary studies}
\label{chap:preliminary_studies}

\par The CFD and CSD solvers, as well as the FSI coupling are thoroughly studied aiming at the achievement of a model that provides the best compromise between accuracy and computation effort, as well as the validation of the solvers and implemented algorithms. Firstly, the generated meshes are investigated according to the span-wise length, the mapping strategy and the first cell height. Then, the available mesh adaption schemes are studied. Secondly, the CSD solver is validated, regarding time dependent external forces and coupled systems. Finally, the FSI coupling is analyzed according to the algorithm responsible for the estimation of displacements, the added mass effect and the coupling scheme itself.

\markboth{CHAPTER 3.$\quad$PREL. STUDIES}{3.1$\quad$CFD STUDIES}
\section{CFD studies}\label{appendix_mesh_adaption}\label{appendix_mesh_studies}

\par The ability of the mesh to provide an accurate solution of the fluid domain in relation to the computational time is thoroughly investigated considering a fixed, as well as a moving airfoil. The three generated meshes, i$.$e$.$, $m{-}L_3^{min}-y^{+}_{min}$, $m{-}L_3^{min}-y^{+}_{max}$ and $m{-}L_3^{max}-y^{+}_{min}$ (see Section \ref{sec:meshes}), are analyzed according to the span-wise length $L_3$, the mapping strategy and the first cell height $\Delta y^{first\,cell}$. The mesh that provides the best comprise between accuracy and required computational time is then utilized to simulate the coupled problem. Finally, the mesh adaption algorithm of the coupled problem is finally investigated, regarding that the TFI, IDW and hybrid IDW-TFI schemes are available.  

\subsection{Investigation of the span-wise length}
\label{sec:study_span_wise_length}
\par A periodic boundary layer is utilized in the $x_3$-direction due to its homogeneity. Since the choice of the span-wise length represents a  compromise between accuracy and numerical effort, the lengths $L_3=0.5\,c$ and $L_3=0.25\,c$ are investigated, as stated in \mbox{Table \ref{table:span_wise_length}}. The former is selected according to the work of Almutari \cite{Almutari_2010}, in which the two-point correlation for the span-wise direction is calculated and is approximately zero, while the latter is based on the work of Schmidt \cite{Schmidt_2016} and Visbal et al.\ \cite{Visbal_2009}.  
\begin{table}[H]
	\centering
	\begin{tabular}{p{3cm} p{2.2cm} p{2cm} p{3.8cm} p{2.5cm}}
		\hline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{\bf{Mesh}}}} & \centering{\bf{Span-wise length (m)}} & \centering{\bf{Mapping strategy}} &\centering{\bf{Maximal iteration number}} & \centering{\bf{Time step size (s)}}\tabularnewline \hline
		\centering{$m{-}L_3^{max}-y^{+}_{min}$} & \centering{$0.50\,c$} & \centering{3} & \centering{$170{,}000$} & \centering{$6\cdot10^{-6}$} \tabularnewline
		\centering{$m{-}L_3^{min}{-}y^+_{min}$} & \centering{$0.25\,c$} & \centering{3} &\centering{$170{,}000$} & \centering{$6\cdot10^{-6}$} \tabularnewline			
		\hline	
	\end{tabular}
	\caption{\label{table:span_wise_length}Comparison of the simulations performed for the meshes with different span-wise lengths $L_3$.}
\end{table}
\par The simulations are performed for a fixed airfoil at a Reynolds number of \mbox{$Re=30{,}000$} utilizing the mapping strategy 3 (see Section \ref{subsubsec:study_mapping_strategy}). The drag and lift coefficients are calculated according to Eqs.\ (\ref{eq:drag_coefficient}) and (\ref{eq:lift_coefficient}). These are time-averaged during a dimensionless time of $t^*=45.6$ and are are summarized in Table \ref{table:drag_lift_coefficients}:
\begin{table}[H]
	\centering
	\begin{tabular}{c p{2.4cm} p{3cm} p{2.4cm} p{3cm}}
		\hline
		\multicolumn{1}{c}{\multirow{3}{*}{\textbf{Mesh}}} & \multicolumn{2}{c}{\textbf{Drag coefficient}} & \multicolumn{2}{c}{\textbf{Lift coefficient}} \tabularnewline
		\cline{2-5}
		& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Mean}}} & \centering{\textbf{Standard deviaton}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Mean}}} & \centering{\textbf{Standard deviaton}} \tabularnewline \hline
		\centering{$m{-}L_3^{max}{-}y^+_{min}$} & \centering{$C_D=0.025$} & \centering{$\sigma_{C_D}=0.001$} & \centering{$C_L=-0.002$} & \centering{$\sigma_{C_L}=0.021$} \tabularnewline
		\centering{$m{-}L_3^{min}{-}y^+_{min}$} & \centering{$C_D=0.025$} & \centering{$\sigma_{C_D}=0.001$} & \centering{$C_L= 0.000$} & \centering{$\sigma_{C_D}=0.022$} \tabularnewline
		\hline
	\end{tabular}
	\caption{\label{table:drag_lift_coefficients}Time-averaged drag and lift coefficients of the $m{-}L_3^{max}{-}y^+_{min}$ and $m{-}L_3^{min}{-}y^+_{min}$ meshes at $Re=30{,}000$.}	
\end{table}
\par The mean and standard deviation values of the averaged drag coefficient are the\break same for both meshes, indicating that the mesh does not influence the\break computation of this aerodynamic property. Since the NACA0012 airfoil is symmetric\break and submitted to an angle of attack of $\alpha=0^\circ$, the expected mean value of the lift\break coefficient is $C_L=0$. A minimal deviation of this value is, however, present when\break the computations are performed with the $m{-}L_3^{max}{-}y^+_{min}$ mesh. Moreover, minor discrepancies of the lift coefficient standard deviations computed by both meshes are also present.
\par The calculated drag coefficients are also quantitatively compared to the experimental results of Sheldahl and Klimas \cite{Sheldahl_1981} for an incidence of $\alpha=0^\circ$, as illustrated in\break \mbox{Fig.\ \ref{fig:comparison_lz}}. These experiments were performed in a wind tunnel for a NACA0012 Eppler model profile at a Reynolds number range of $1\cdot10^4\leq Re\leq1\cdot10^7$ and an\break incidence range of \mbox{$0^\circ \leq \alpha \leq 180^\circ$}. Since the simulated airfoil profile (see NASA \cite{NASA_2016}) is slightly different from the NACA0012 Eppler model profile (see Fig.\ \ref{fig:comparison_NACA0012_NASA_Eppler}), the\break results achieved by the simulations are overestimated compared to the experimental results.  
\par Due to the minor differences in the results achieved by both simulated meshes\break ($m{-}L_3^{max}{-}y^+_{min}$ and $m{-}L_3^{min}{-}y^+_{min}$), even the mesh with the the smallest span-wise\break length is able to accurately simulate the fluid domain. Moreover, the $m{-}L_3^{min}{-}y^+_{min}$ mesh uses only $53.05\%$ of the required computational time of the $m{-}L_3^{max}{-}y^+_{min}$ grid. Therefore the meshes with a span-wise length of $L_3=0.25\,c$ are applied to compute the FSI cases. 
\begin{figure}[H]
	\centering
	\includegraphics[width=0.6\textwidth]{\FigPath/Masterarbeit/comparison_cd_lz.pdf} 
	\caption{Drag coefficients of the airfoil at an incidence of $\alpha=0^\circ$. Current work: NASA NACA0012 \cite{NASA_2016}. \mbox{Sheldahl and Klimas \cite{Sheldahl_1981}}: NACA0012 Eppler model.}
	\label{fig:comparison_lz}
\end{figure} 
\begin{figure}[H]
	\centering
	\includegraphics[width=0.6\textwidth]{\FigPath/Masterarbeit/geometry_NACA0012_NACA0012_Eppler.pdf} 
	\caption{NASA NACA0012 \cite{NASA_2016} profile used in the current work and NACA0012 Eppler model profile from Sheldahl and Klimas \cite{Sheldahl_1981}.}
	\label{fig:comparison_NACA0012_NASA_Eppler}
\end{figure}

\subsection{Investigation of the mapping strategy}
\label{subsubsec:study_mapping_strategy}
\par The twelve geometrical blocks generated by ICEM CFD are divided and combined in a process called mapping. This aims at the creation of as cubic as possible parallel blocks in order to guarantee the fastest computation of the flow domain. Each parallel block is solved by a different processor with information exchange occurring only at its faces, so that the computation of all blocks can be performed at the same time (parallel computing).
\par Four mapping strategies for the $m{-}L_3^{min}{-}y^+_{min}$ mesh are investigated, regarding that cubic parallel blocks with 70$,$000 control volumes are aimed. Moreover, the blocks are not divided in the $\eta$-direction in order to avoid numerical damping of the plunge movement due to the stiffening of block boundaries. Simulations for the fluid-structure interaction of a NACA0012 airfoil with two degrees of freedom (pitch and plunge) are carried out for a Reynolds number of $Re=30{,}000$ and a linear stiffness of $k_{l,\,2}=144\,N{\cdot}m^{-1}$. Thousand time steps ($n=1000$) are computed in order to compare the efficiency of the different mappings. The properties of the applied mapping strategies are compared in Table \ref{table:mapping_strategy}: 
\begin{table}[H]
	\centering
	\begin{tabular}{p{1.69cm} p{2.2cm} p{3.5cm} p{1.9cm} p{3.9cm}}
		\hline
		\multicolumn{1}{c}{\multirow{3}{1.69cm}{\centering{\bf{Mapping strategy}}}} & \multicolumn{1}{c}{\multirow{3}{2.2cm}{\centering{\bf{Required processors}}}} & \centering{\bf{Averaged control volumes per processor}} &\centering{\bf{Load-balancing efficiency}} & \centering{\bf{Averaged computational time per time step}} \tabularnewline \hline
		\centering{1} & \centering{18} & \centering{59$,$200} & \centering{54.81\%} & \centering{0.93 s} \tabularnewline
		\centering{2} & \centering{23} & \centering{46$,$330}&\centering{64.35\%} & \centering{0.90 s} \tabularnewline
		\centering{3} & \centering{13} & \centering{81$,$969} & \centering{75.90\%} & \centering{0.72 s} \tabularnewline
		\centering{4} & \centering{15} & \centering{71$,$040}& \centering{87.70\%} & \centering{0.72 s} \tabularnewline				
		\hline	
	\end{tabular}
	\caption{\label{table:mapping_strategy}Comparison of the mapping strategies.}
\end{table}
\par Load-balancing efficiency indicates the effectiveness of the work (computation of the whole fluid domain) division into separate tasks performed by each processor. Generally, the higher the load-balancing efficiency, the lower the required computational time, since the processor idle time is optimized. Although the mapping strategy 4 has the highest load-balancing efficiency, the required computational time is equal to the one achieved with mapping strategy 3. Therefore, the processor idle time, the information exchange between processors and the computation of the parallel blocks are optimized for the mapping \mbox{strategies 3 and 4}. Nonetheless, strategy 4 is utilized to  investigate the fluid-structure interaction between air and NACA0012 airfoil due to the highest load-balancing efficiency.
\begin{figure}[H]
	\centering
	\subfigure[Top view.]{\includegraphics[width=0.44\textwidth]{\FigPath/Masterarbeit/mapping_grob_grid_1pt8e-5_lz_0pt25_suction_side.pdf}\label{fig:blocking_top_view}}\\
	\centering	
	\subfigure[Front view.]{\includegraphics[width=0.44\textwidth]{\FigPath/Masterarbeit/mapping_grob_grid_1pt8e-5_lz_0pt25.pdf} \label{fig:blocking_front_view}}
\end{figure}
\begin{figure}[H]
	\centering
	\subfigure[Bottom view.]{\includegraphics[width=0.44\textwidth]{\FigPath/Masterarbeit/mapping_grob_grid_1pt8e-5_lz_0pt25_pressure_side.pdf}\label{fig:blocking_bottom_view}}
	\caption{Parallel blocks of the mapping strategy 4.}
	\label{fig:mapping_grid}
\end{figure} 
\par The distribution of the parallel blocks of mapping strategy 4 is illustrated in \mbox{Fig.\ \ref{fig:mapping_grid}}. Each color represent the blocks computed by a determined processor, totalizing a number of 15 processors for the computation of the whole fluid domain.


\subsection{Investigation of the first cell height}
\label{sec:investigation_first_cell_height}
\par The non-slip condition on the airfoil surface is responsible for the generation of a velocity gradient on the cells located at this interface. In order to guarantee the accuracy of the wall-resolved LES, the gradients present on a cell must be small. Therefore, the maximal allowed height of the cells in contact with non-slip walls is limited. 
\par Since this mesh property is directly related to the maximal applicable time step used to obtain a converged solution, the first cell height is defined by the best compromise between accuracy and required computational time. Therefore, two meshes with the same number of control volumes, the same mapping strategy and different first cell heights are compared, as illustrated in Table \ref{table:first_cell_height}. The simulations are performed for a fixed airfoil at a Reynolds number of $Re=30{,}000$ until a dimensionless time of $t^*=t\,u_{1,\,in}/c=200$ is achieved. Thereto, a total of $n=450{,}000$ and $n=750{,}000$ iterations are computed for the $m{-}L_3^{min}-y^{+}_{max}$ and $m{-}L_3^{min}{-}y^+_{min}$ meshes, respectively. The time-averaging process is started when the flow is completely developed, i$.$e$.$, after $t^*_{init}=67$. 
\begin{table}[H]
	\centering
	\begin{tabular}{p{3cm} p{2.09cm} p{2.5cm} p{2.3cm} p{2.8cm}}
		\hline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{\bf{Mesh}}}} & \centering{\bf{Span-wise width (m)}} & \centering{\bf{Mapping strategy}} &\centering{\bf{First cell height (m)}} & \centering{\bf{Time step size (s)}}\tabularnewline \hline
		\centering{$m{-}L_3^{min}-y^{+}_{max}$} & \centering{$0.25\,c$} & \centering{3} & \centering{$5.0\cdot10^{-5}$} & \centering{$1\cdot10^{-5}$} \tabularnewline
		\centering{$m{-}L_3^{min}{-}y^+_{min}$} & \centering{$0.25\,c$} & \centering{3} &\centering{$1.8\cdot10^{-5}$} & \centering{$6\cdot10^{-6}$} \tabularnewline			
		\hline	
	\end{tabular}
	\caption{\label{table:first_cell_height}Comparison of the meshes with different first cell heights.}
\end{table}
\par The simulation with the $m{-}L_3^{min}-y^{+}_{max}$ mesh is approximately two times faster than the one with the $m{-}L_3^{min}-y^{+}_{max}$ grid. The accuracy of the simulations is compared through the calculation of the time-averaged dimensionless wall distances $y^+$, as illustrated in \mbox{Fig.\ \ref{fig:y_plus_lz_0pr25}}. 
\par The maximal dimensionless wall distance is achieved for the \mbox{$m{-}L_3^{min}-y^{+}_{max}$} mesh. Since these values are contained in a range of $0\leq y^+\leq 1.4$, the viscous sublayer can still be solved and only minor velocity gradients are present on the cells. Hence, the $m{-}L_3^{min}-y^{+}_{max}$ grid is utilized for the FSI simulations, as it represents the best compromise between accuracy and required computational time.
\begin{figure}[H]
	\centering
	\subfigure[$m{-}L_3^{min}-y^{+}_{max}$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/y_plus_grob_grid_5e-5_wall_distance_lz_0pt25.pdf} \label{fig:y_plus_5}}\hfill
	\subfigure[$m{-}L_3^{min}{-}y^+_{min}$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/y_plus_grob_grid_1pt8e-5_wall_distance_lz_0pt25.pdf}\label{fig:y_plus_1pt8}}\hfill
	\caption{Time-averaged dimensionless wall distances of the meshes with $L_3=0.25\,c$.}
	\label{fig:y_plus_lz_0pr25}
\end{figure}  


\subsection{Investigation of the mesh adaption algorithm}
\label{appendix_mesh_adaption}

\par The $m{-}L_3^{min}-y^{+}_{max}$ mesh with the mapping strategy 4 is applied in order to thoroughly analyze the available mesh adaption algorithms. Since the largest displacements are achieved for the test case characterized by extremely small linear and torsional stiffnesses (see \mbox{Section \ref{subsec:inv_great_airfoil_disp})}, the investigations are based on the maximal airfoil response achieved by this computation.
\par Various simulations utilizing distinct mesh adaption algorithms, as well as various re-meshing parameters are performed in order to establish the method that provides the better quality of the mesh while requiring the smallest computational time. These test cases are simulated considering only a translational displacement of $X_2=0.3\,\text{m}$, which is slightly greater than the maximal translational displacement achieved by the coupled simulation with the TFI re-meshing algorithm (see Section \ref{subsec:inv_great_airfoil_disp}), since the rotational displacement is not considered. The latter is not thoroughly studied, since the cause of the numerical difficulties for angles up to $\varphi_3=49.42^\circ$ is actually the maintenance of the height of the cells located on the airfoil surface and not the preservation of the mesh orthogonality (see Section \ref{subsec:inv_great_airfoil_disp}).
\par The translational displacement of $X_2=0.3\,\text{m}$ is gradually applied as a boundary condition according to Eq.\ (\ref{eq:disp_func}), regarding that $A=0.3\,m$. This procedure must be undertaken, since the IDW and hybrid IDW-TFI algorithms adapt the mesh also in relation to the last time step. A total of $n=1{,}000$ time steps are computed with a time step size of \mbox{$\Delta t=1{\cdot}10^{-3}\,\text{s}$}. The fluid domain is not solved and therefore the required computational time represents only the time needed to adapt the mesh in relation to the new boundaries.  
\begin{equation}
\label{eq:disp_func}
X_{2,\,mesh\,adapt.}=A\,t
\end{equation}
\par The results achieved for all test cases are summarized in Table \ref{table:comp_re_meshing_algorithms}, regarding that the TFI, IDW and hybrid IDW-TFI re-meshing algorithms are examined and that the first cell height $\Delta y^{first\,cell}$ is indicated as $H$ for the sake of simplicity. Although the former algorithm is not applicable for this test case (see \mbox{Section \ref{subsec:inv_great_airfoil_disp})}, this is also computed in order to enable a comparison of the required computational time and the mesh quality. The weighting function utilized to realize the interpolation of the IDW and IDW-TFI methods (see Section \ref{subsubsec:idw_tfi}), can be adapted according to the parameters $\alpha_{fxd}$ and $\alpha_{mv}$, regarding that their increase lead to a stiffer mesh adaption (see \mbox{Sen et al.\ \cite{Sen_2017})}. The former describes the adaption of the fixed boundaries, i$.$e$.$, inlet, outlet, symmetry and periodic while the latter describes the adaption of the moving boundaries, that is, the airfoil wall boundary submitted to the fluid-structure interaction.
\begin{table}[H]
	\centering
	\begin{tabular}{p{3cm} p{3cm} p{3.5cm} p{3.5cm}}
		\hline
		\multicolumn{2}{c}{\bf{Re-meshing}} & \multicolumn{1}{c}{\multirow{2}{3cm}{\centering{\bf{Computational time (h)}}}} & \multicolumn{1}{c}{\multirow{2}{2.5cm}{\centering{\bf{First cell height (m)}}}} \tabularnewline\cline{1-2}
		\centering{\bf{Method}} & \centering{\bf{Parameters}} & & \tabularnewline \hline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{TFI}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{-}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{0.020}}} & \centering{$H\geq2.8{\cdot}10^{-5}$ $H\leq 7.0{\cdot}10^{-5}$} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{IDW}}} & \centering{$\alpha_{fxd}=0.1$ $\alpha_{mv}=0.3$} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{9.639}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.05$ $\alpha_{mv}=0.3$} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{3.035}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.1$ $\alpha_{mv}=0.3$} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{3.030}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.13$ $\alpha_{mv}=0.3$} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{3.031}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.15$ $\alpha_{mv}=0.3$} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{3.053}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.2$ $\alpha_{mv}=0.3$} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{3.034}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{2.3cm}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.5$ $\alpha_{mv}=0.3$} & \multicolumn{1}{c}{\multirow{2}{3cm}{\centering{3.032}}} & \multicolumn{1}{c}{\multirow{2}{2.5cm}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.1$ $\alpha_{mv}=0.1$} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{3.033}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.13$ $\alpha_{mv}=0.1$} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{3.069}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
%	\end{tabular}
%\end{table}	
%\begin{table}[H]
%	\centering
%	\begin{tabular}{p{3cm} p{3cm} p{3.5cm} p{3.5cm}}
		\multicolumn{1}{c}{\multirow{2}{3cm}{\centering{IDW-TFI}}} & \centering{$\alpha_{fxd}=0.13$ $\alpha_{mv}=0.5$} & \multicolumn{1}{c}{\multirow{2}{3.5cm}{\centering{3.031}}} & \multicolumn{1}{c}{\multirow{2}{3.5cm}{\centering{$H=5.0{\cdot}10^{-5}$}}} \tabularnewline
		\hline
	\end{tabular}
	\caption{\label{table:comp_re_meshing_algorithms}Comparison of the re-meshing algorithms: Translational displacement of \mbox{$X_2=0.3\,m$}.}
\end{table}
\par The smallest computational time is achieved utilizing the TFI algorithm, which adapted mesh is illustrated in Fig.\ \ref{fig:mesh_tfi_re_meshing} for the considered displacement, regarding that one out ot two mesh lines is displayed for both the $\xi$-axis on the front domain and the $\eta$-axis on the whole fluid domain. The mesh orthogonality is only not deeply affected due to the fact that no airfoil rotation is present. The first cell height is not maintained, varying between $2.8{\cdot}10^{-5}\,\text{m}\leq \Delta y^{first\,cell}\leq 7.0{\cdot}10^{-5}\,\text{m}$ for the control volumes located on the airfoil surface,\break regarding a initial value of $\Delta y^{first\,cell}= 5.0{\cdot}10^{-5}\,m$. The cell height is also not maintained at the fixed boundaries, i$.$e$.$, the control volumes located at the bottom of the fluid domain are larger than the ones located at the top. Moreover, degenerated cells are created at the\break trailing edge. Therefore, the utilization of this adaptation method always leads to numerical difficulties if large displacements are observed, even if no rotation is present.
\begin{figure}[H]
	\centering
	\subfigure[Adapted mesh - Overall view.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/grid_y_disp_tfi.pdf} \label{fig:mesh_overall_tfi_re_meshing}}\hfill
	\subfigure[Adapted mesh - Focus on the trailing edge.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/grid_y_disp_tfi_zoom_trailing_edge.pdf} \label{fig:mesh_trailing_edge_tfi_re_meshing}}\hfill
	\caption{TFI algorithm: Mesh adaption considering a translational displacement of \mbox{$X_2=0.3\,\text{m}$}.}
	\label{fig:mesh_tfi_re_meshing}
\end{figure}
\par The IDW  and hybrid IDW-TFI methods are characterized by the maintenance of the first cell height, i$.$e$.$, $\Delta y^{first\,cell}=5{\cdot}10^{-5}\,\text{m}$. Since the required computational time of the former method is about 3.2 and 481.9 times higher than the hybrid IDW-TFI and TFI algorithms while the achieved mesh quality is exactly the same of the hybrid method, the IDW scheme is not considered for further studies.
\par Nine different combinations of the parameters that determine the weighting function of the fixed and the movable boundaries, i$.$e$.$, $\alpha_{fxd}$ and $\alpha_{mv}$, are investigated for the hybrid IDW-TFI algorithm. Since the best mesh quality is achieved for the parameters $\alpha_{fxd}=\alpha_{mv}=0.1$, the mesh adapted utilizing them is illustrated in Fig.\ \ref{fig:mesh_idw_tfi_re_meshing}.
\par The problems generated by the TFI algorithm are overcome through the utilization of this method, i$.$e$.$, no degenerated cells are created at the trailing edge, as well as the first cell height is maintained for all cells located on the airfoil surface, enabling the computation with constant time step sizes. Moreover, the required computational time is reasonable considering the one needed by the IDW method. Although the achieved skew metric quality is low, i$.$e$.$, $f_{skew}\geq0.599$, Fig.\ \ref{fig:mesh_skew_idw_tfi_re_meshing} illustrates that the cells with lower quality are located distant from the airfoil, which does not lead to accuracy problems since the critical flow phenomena occur near the airfoil.
\begin{figure}[H]
	\centering
	\subfigure[Adapted mesh - Overall view.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/grid_y_disp_idw_tfi_0pt1_0pt1.pdf} \label{fig:mesh_overall_idw_tfi_re-meshing}}\hfill
	\subfigure[Adapted mesh: Focus on the trailing edge.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/grid_y_disp_idw_tfi_0pt1_0pt1_zoom_trailing_edge.pdf}\label{fig:mesh_trailing_edge_idw_tfi_re_meshing}}\hfill
	\caption{Hybrid IDW-TFI algorithm with $\alpha_{fxd}=\alpha_{mv}=0.1$: Mesh adaption considering a translational displacement of $X_2=0.3\,\text{m}$.}
	\label{fig:mesh_idw_tfi_re_meshing}
\end{figure}

\begin{figure}[H]
	\centering
	\centering
	\includegraphics[scale=0.85,draft=\drafttype]{\FigPath/Masterarbeit/grid_skew_y_disp_idw_tfi_0pt1_0pt1.pdf}
	\caption{\label{fig:mesh_skew_idw_tfi_re_meshing}Hybrid IDW-TFI algorithm with $\alpha_{fxd}=\alpha_{mv}=0.1$: Mesh quality considering a translational displacement of $X_2=0.3\,\text{m}$.}
\end{figure}

\subsection{Conclusions}
\label{sec:conclusions_mesh_investigations}
\par The thorough investigations of the three generated meshes and the four\break mapping strategies pointed out that the minimal computational time is achieved with the \mbox{$m{-}L_3^{min}-y^{+}_{max}$} mesh while utilizing the mapping strategy 4. Since this configuration also provides an accurate computation, this is utilized to approximate the solution of the coupled test cases.
\par Moreover, the IDW-TFI method is chosen to further simulate cases characterized by large airfoil translational and rotational displacements. Although this requires a higher computational time than the TFI method, this does not lead to numerical difficulties due to the maintenance of the height of the cells located on the airfoil surface and therefore can also be utilized for large rotations without the generation of cells with negative volumes. Furthermore, the parameters $\alpha_{fxd}=\alpha_{mv}=0.1$ are applied due to the generation of the best mesh quality considering the orthogonality of the grid.  



\markboth{CHAPTER 3.$\quad$PRELIMINARY STUDIES}{3.1$\quad$CSD STUDIES}
\section{CSD studies}\label{appendix_validation_CSD}

\par In the case of fluid-structure interaction between flow and NACA0012 profile with two degrees of freedom (pitch and plunge), the external forces acting on the rigid airfoil, i$.$e$.$, the fluid forces, can be time dependent. Since Viets \cite{Viets_2013} validated the applied in-house rigid movement solver (see Section \ref{sec:CSD}) only for the case of a constant external force, this software is also verified regarding systems with a time dependent external force and a coupled translational and rotational motion.

\subsection{System under rotating unbalance}
\label{sec:rotating_unbalance}
\par Rotating unbalance is one of the main causes of vibration in rotating machinery, such as turbines and rotors. A simplified model, as illustrated in Fig.\ \ref{fig:rotating_unbalance}, is utilized in order to compare the analytical and numerical results. 
\begin{figure}[H]
	\centering
	\includegraphics[scale=0.53,draft=\drafttype]{\FigPath/Masterarbeit/rotating_unbalance.pdf}
	\caption{\label{fig:rotating_unbalance}System under rotating unbalance.}
\end{figure}
\par Two eccentric masses $m_{ex}/2$ with a determined eccentricity $e_{m_{ex}}$ rotate with the same constant angular frequency $\omega$ in opposite directions. The generated centrifugal force ($m_{ex}\,e_{m_{ex}}\,\omega^2$) is decomposed into the horizontal and vertical components. While the former is canceled due to the rotation of the eccentric masses in opposite directions, the latter contributes to the vibration of the machine \cite{Rao_2011}. Therefore, displacements of the rigid body occurs only in the vertical direction.
\par Equations (\ref{eq:rotating_unbalance_undamped}) and (\ref{eq:rotating_unbalance_damped}) describe the motion of the body for the undamped and damped cases (see Rao \cite{Rao_2011}), respectively. $m$, $c_l$, $k_l$ and $t$ represent the total mass of the system, the linear damping coefficient, the linear spring stiffness and the time, respectively. $\ddot{X}$, $\dot{X}$ and $X$ are the translational acceleration, velocity and displacement of the body (the subscripted $t$ and directional index $i=2$, for instance in $X_{t,\,2}$, are omitted for the sake of brevity). The left side of the equation stands for the internal forces while the right one represents the time dependent external force caused by the rotation of the eccentric masses.
\begin{eqnarray}
\label{eq:rotating_unbalance_undamped}
m\,\ddot{X}+k_l\,X=m_{ex}\,e_{m_{ex}}\,\omega^2\,sin(\omega t)\\
\label{eq:rotating_unbalance_damped}
m\,\ddot{X}+c_l\,\dot{X}+k_l\,X=m_{ex}\,e_{m_{ex}}\,\omega^2\,sin(\omega t)
\end{eqnarray} 
\par The analytical solutions of these differential equations are based on the sum of the homogeneous and the particular solutions (see Rao \cite{Rao_2011}). Equations (\ref{eq:rotating_unbalance_solution_undamped}) and (\ref{eq:rotating_unbalance_solution_underdamped}) represent respectively the solution of the undamped and the underdamped (D\,<\,1) systems:
\begin{eqnarray}
\label{eq:rotating_unbalance_solution_undamped}
X(t)&=&X_0\,cos(\omega_n t + \phi_1)+X_0\,sin(\omega t + \phi_2), \\\nonumber
\label{eq:rotating_unbalance_solution_underdamped}
X(t)&=&e^{-D\,\omega_n\,t}\,[X_0\,cos(\omega_n t+\phi_1)+D\,X_0\,sin(\omega_n t+\phi_1)]\\&+&X_0\,sin(\omega t+\phi_2).
\end{eqnarray}
\par $X_0$ represents a characteristic amplitude and is calculated according to Eq.\ (\ref{eq:rotating_unbalance_amplitude}). The damping ratio $D$ is a relation between the utilized damping constant $c_l$ and the critical damping coefficient $c_c$, as per Eq.\ (\ref{eq:damping_ratio}). The natural frequency $w_n$ is a relation between the spring stiffness $k_l$ and the total mass of the system $m$ (see Eq.\ (\ref{eq:natural_frequency})). $\phi_1$ and $\phi_2$ represent the phase angles. These are calculated through a system of equations, which are generated by the application of the initial conditions in the governing equation \mbox{(either Eq.\ (\ref{eq:rotating_unbalance_undamped}) or Eq.\ (\ref{eq:rotating_unbalance_damped}))}. The current analysis utilizes a zero displacement and zero velocity as initial conditions, i$.$e$.$, $X(t=0)=0$ and $\dot{X}(t=0)=0$.
\begin{eqnarray}
\label{eq:rotating_unbalance_amplitude}
X_0&=&\frac{m_{ex}\,e_{m_{ex}}\,\omega^2}{\sqrt{(k_l-m\,\omega^2)^2+(c_l\,\omega)^2}}\\
\label{eq:damping_ratio}
D&=&\frac{c_l}{c_c}=\frac{c_l}{2\sqrt{k\,m}}\\
\label{eq:natural_frequency}
\omega_n&=&\sqrt{\frac{k_l}{m}}
\end{eqnarray}
\par When the angular frequency of the eccentric masses $\omega$ and the natural frequency $\omega_n$ have the same value, resonance occurs. The current analysis is performed for an angular frequency near the natural frequency for damping ratios of $D=0$ and $D=0.25$. The setup of these test cases is presented in Table \ref{table:rotating_unbalance_variables}, while the setup of the analytical solution is indicated in \mbox{Table \ref{table:rotating_unbalance_analytical}}:
\begin{table}[H]
	\centering
	\begin{tabular}{p{3cm} p{3.5cm} p{3cm}}
		\hline
		{\bf{Variable}} & \bf{Undamped case} & \bf{Damped case} \tabularnewline \hline
		$m\,(\text{kg})$ &\multicolumn{1}{c}{10} & \multicolumn{1}{c}{10}  \tabularnewline
		$c_l\,(\text{N}{\cdot}\text{s}{\cdot}\text{m}^{-1})$ & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{25} \tabularnewline
		$D$& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0.25} \tabularnewline
		$k_l\,(\text{N}{\cdot}\text{m}^{-1})$& \multicolumn{1}{c}{250}& \multicolumn{1}{c}{250} \tabularnewline
		$m_{ex}\,(\text{kg})$& \multicolumn{1}{c}{1}& \multicolumn{1}{c}{1} \tabularnewline
		$e_{m_{ex}}\,(\text{m})$& \centering{0.45}& \centering{0.45} \tabularnewline	
	\end{tabular}
\end{table}
\begin{table}[H]
	\centering
	\begin{tabular}{p{3cm} p{3.5cm} p{3cm}}
		$\omega\,(\text{rad}{\cdot}\text{s}^{-1})$& \centering{4.5} & \centering{4.5}  \tabularnewline
		$\omega_n\,(1{\cdot}\text{s}^{-1})$& \centering{5}& \centering{5} \tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:rotating_unbalance_variables}Setup of the systems submitted to rotating unbalance.}
\end{table}
\begin{table}[H]
	\centering
	\begin{tabular}{l c c}
		\hline
		\multicolumn{1}{c}{\bf{Variable}} & \bf{Undamped case} & \bf{Damped case} \tabularnewline \hline
		$X_0\,(\text{m})$& 0.182& 0.075 \tabularnewline
		$\phi_1\,(\text{rad})$& $\pi$& -0.133 \tabularnewline
		$\phi_2\,(\text{rad})$& $\pi/2$ & -1.438 \tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:rotating_unbalance_analytical}Setup of the analytical solutions - Rotating unbalance test case.}
\end{table}
\par Two numerical simulations are performed for each system configuration: One with the ode45 solver of Matlab Simulink and other with the rigid movement solver implemented by Viets \cite{Viets_2013}. The former is based on the Dormand-Prince method \cite{Dormand_1980}, which is a fifth-order accuracy explicit variable-step solver applicable for models with continuous states. Therefore, it is suitable for mass-spring-damper systems. The specified minimal and maximal step sizes are $\Delta t_{min}=10^{-4}\,\text{s}$ and $\Delta t_{max}=10^{-3}\,\text{s}$, regarding that the time step size is reduced or increased among this interval using a local error control to achieve the specified tolerance \cite{Matlab_2015}, i$.$e$.$, $10^{-3}$. The rigid movement solver (see Section \ref{sec:CSD}) applies the implicit standard Newmark time discretization method with a time step size of $\Delta t=10^{-3}\,\text{s}$, since this is the largest value that does not influence the solution. The system is allowed to oscillate \mbox{only in one degree of freedom at a time.}
\par The comparison between analytical and numerical solutions are presented in\break \mbox{Fig.\ \ref{fig:disp_rotating_unbalance}} for both undamped and damped cases. All six degrees of freedom are tested and deliver the same solution.   
\begin{figure}[H]
	\centering
	\subfigure[Undamped system $D=0$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/test_rotating_unbalance_D0.pdf}\label{fig:disp_rotating_unbalance_undamped}}\hfill
	\subfigure[Damped system $D=0.25$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/test_rotating_unbalance_D0pt25.pdf} \label{fig:disp_rotating_unbalance_damped}}\hfill
	\caption{Displacements of the undamped and damped rotating unbalance cases: Numerical and analytical solutions.}
	\label{fig:disp_rotating_unbalance}
\end{figure}
\par The numerical solutions achieved with the Matlab Simulink and the rigid movement solvers deliver exactly the same results. Although the utilized initial conditions and the maximal amplitude are the same for both numerical and analytical solutions, a small discrepancy is present in the beginning of the oscillation for the undamped case and a minimal phase shift is present for the damped case. Since the angular frequency of the eccentric masses are near the resonance frequency, a considerable amplitude of oscillation is achieved for $D=0$ and the damping coefficient is responsible for the constant amplitude achieved for $D=0.25$.
  

\subsection{System under coupled translation and rotation}
\label{sec:coupled_translation_rotation}

\par The disc of the disc-spring system rolls over its instantaneous center of rotation $S$ without sliding (see Fig.\ \ref{fig:coupled_rotation_translation}). Its movement is characterized by a coupled translational and rotational motion, since the instantaneous center of rotation does not coincide with the center of mass $\mbox{CM}$.
\begin{figure}[H]
	\centering
	\includegraphics[scale=0.8,draft=\drafttype]{\FigPath/Masterarbeit/coupled_rotation_translation.pdf}
	\caption{\label{fig:coupled_rotation_translation}System with coupled rotation and translation.}
\end{figure}
\par The governing equations for the rotational and translational motions (see Eqs.\ (\ref{eq:disc_spring_system_translation}) and (\ref{eq:disc_spring_system_rotation})) are acquired through Euler's equation of motion for a rotation outside the center of mass (see Gere \cite{Gere_2004}) and through the relation between the rotational and translational motions (see Rao \cite{Rao_2011}). $\ddot{\varphi}$ and $\varphi$ represent the angular acceleration and displacement while $k_l$, $m$, $r$ and $X$ represent respectively the linear spring stiffness, the disc mass, the disc radius and the translational displacement. 
\begin{eqnarray}
\label{eq:disc_spring_system_rotation}
\ddot{\varphi}+\frac{2\,k_l}{3\,m}\varphi&=&0\\
\label{eq:disc_spring_system_translation}
X&=&r\,\varphi
\end{eqnarray}
\par The setup of the present test case is described in Table \ref{table:coupled_rotation_translation} for both the rigid movement solver and the ode45 solver of Matlab Simulink. The initial conditions are set to \mbox{$\varphi (t=0)=1$} and $\dot{\varphi} (t=0)=0$.
\begin{table}[H]
	\centering
	\begin{tabular}{p{3.5cm} p{4.5cm} p{4cm}}
		\hline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{\bf{Variable}}}} & \centering{\bf{Rigid movement solver}} & \centering{\bf{Matlab Simulink ode45 solver}} \tabularnewline \hline
		$m\,(\text{kg})$& \centering{1}& \centering{1} \tabularnewline
		$r\,(\text{m})$& \centering{0.5} & \centering{0.5} \tabularnewline
		$k_l\,(\text{N}{\cdot}\text{m}^{-1})$& \centering{6} & \centering{6} \tabularnewline
		$\Delta t\,(\text{s})$ & \centering{$10^{-3}$} & \centering{$10^{-4}\leq \Delta t\leq 10^{-3}$} \tabularnewline
		Time discretization method& \multicolumn{1}{c}{\multirow{2}{*}{\centering{Standard Newmark}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{Dormand-Prince}}} \tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:coupled_rotation_translation}Setup of the numerical solutions - Coupled rotation and translation test case.}
\end{table}
\par For the simulations performed with the rigid movement solver, two degrees of freedom (one translational and other rotational) are tested at a time and all nine possible combinations deliver the same results. The rotational and translational oscillations are illustrated in Fig.\ \ref{fig:coupled_system_oscillation}. The results achieved with the ode45 solver of the Matlab Simulink and with the in-house rigid movement solver are exactly the same. 
\begin{figure}[H]
	\centering
	\subfigure[Rotational displacement.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/test_coupled_rotation.pdf} \label{fig:coupled_system_rotation}}\hfill
	\subfigure[Translation displacement.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/test_coupled_translation.pdf}\label{fig:coupled_system_translation}}\hfill
	\caption{Translational and rotational displacements of the coupled system.}
	\label{fig:coupled_system_oscillation}
\end{figure}

\subsection{Conclusions}
\label{sec:conclusions_CSD_validation}
\par The executed test cases assured the accuracy of the rigid movement solver implemented by Viets \cite{Viets_2013} through comparisons with reference analytical and numerical solutions. The former is based on Rao \cite{Rao_2011} and applicable only for the rotating unbalance test case, while the latter is achieved through simulations performed in the reference solver ode45 from Matlab Simulink. Due to the great correspondence between all comparable solutions, the rigid movement code is then validated also for problems characterized by time dependent external forces and coupled motions. Therefore, it should be able to accurately compute the structural response of the NACA0012 airfoil when it is submitted to fluid-structure interaction. 


\markboth{CHAPTER 3.$\quad$PRELIMINARY STUDIES}{3.1$\quad$FSI COUPLING STUDIES}
\section{FSI coupling studies}\label{appendix_FSI_coupling_studies}

\par The algorithm utilized for the estimation of displacements, as well as the added mass effect and the coupling method are thoroughly analyzed. Since the utilization of the estimation of displacements together with a loosely coupled algorithm requires the smallest computational time, the studies primarily aim at the analysis of the accuracy of this method through a comparison with other algorithms. Thereby, the best compromise between accuracy and numerical effort can be determined and further utilized for the FSI simulations.

\subsection{Investigation of the estimation of displacements}
\label{subsec:investigation_estimation_displacement}

\par The linear extrapolation of the displacements is implemented in order to improve the convergence properties and therefore to reduce the required computational time. Two strong coupled simulations of the fluid-structure interaction between NACA0012 airfoil and flow are executed for the $m{-}L_3^{min}{-}y_{max}^+$ mesh utilizing the mapping strategy 4. The FSI is computed for two degrees of freedom (pitch and plunge) with linear and  torsional stiffnesses of $k_{l,\,2}=144\,\text{N}{\cdot}\text{m}^{-1}$ and $k_{t,\,3}=0.3832\,\text{N}{\cdot}\text{m}{\cdot}\text{rad}^{-1}$, respectively. Moreover, the chord Reynolds number is $Re=30{,}000$, the FSI convergence criterion is $\epsilon_{FSI,\,disp}<1{\cdot}10^{-6}$ and the computation runs until a dimensionless time of $t^*=4.47$ is achieved. Further properties of these simulations are summarized in Table \ref{table:comp_est_disp}:
\begin{table}[H]
	\centering
	\begin{tabular}{p{3cm} p{2.7cm} p{2.5cm} p{3cm} p{2cm}}
		\hline
		\multicolumn{1}{c}{\multirow{3}{*}{\centering{\bf{Mesh}}}} & \centering{\bf{Estimation of displacement}} & \centering{\bf{Maximal iteration number}} & \centering{\bf{Maximal number of sub-iterations}} & \centering{\bf{Time step size (s)}}\tabularnewline \hline
		\centering{$m{-}L_3^{min}{-}y^{+}_{max}$} & \centering{Yes} & \centering{$10{,}000$} & \centering{20} & \centering{$1\cdot10^{-5}$} \tabularnewline
		\centering{$m{-}L_3^{min}{-}y^+_{max}$} & \centering{No} & \centering{$14{,}286$} &\centering{20} & \centering{$7\cdot10^{-6}$} \tabularnewline			
		\hline	
	\end{tabular}
	\caption{\label{table:comp_est_disp}Simulation properties of the test cases aimed at the study of the advantages achieved by the  utilization of the prediction of the displacements.}
\end{table}
\par The simulation without prediction of the displacements requires a smaller time step, otherwise the computation of the FSI case diverges since the utilization of 20 sub-iterations is not enough to obtain a converged result for each time step.  Therefore, in order to achieve the same dimensionless time step, this simulation requires also the calculation of a greater number of iterations, increasing the necessary numerical effort.
\par After the initialization phase, the simulation that utilizes the estimation of displacements generally requires the calculation of only two sub-iterations in order to converge, while the simulation that does not predict the displacements computes frequently all twenty sub-iterations without always achieving the convergence criterion, as illustrated in Figs.\ \ref{fig:used_iterout_comparison} and \ref{fig:residuum_convergence_comparison}. Although the convergence criterion is $\epsilon_{FSI,\,disp}<1{\cdot}10^{-6}$, many time steps of the simulations with the prediction of the displacements achieve residua in the order of magnitude of $\epsilon_{FSI,\,disp}\leq\mathcal{O}(10^{-7})$. This occurs, since the previous sub-iteration $n_{FSI}$ has not yet achieved the convergence criterion, while the current sub-iteration $n_{FSI}+1$ achieves it and also reduces the residuum of displacement up to three orders of magnitude. 
\begin{figure}[H]
	\centering
	\subfigure[Simulation with estimation of displacement.]{\includegraphics[width=0.495\textwidth]{\FigPath/Masterarbeit/used_it_itout20_est_disp.pdf} \label{fig:used_iterout_est_disp}}\hfill
	\subfigure[Simulation without estimation of displacement.]{\includegraphics[width=0.495\textwidth]{\FigPath/Masterarbeit/used_it_itout20_no_est_disp.pdf}\label{fig:used_iterout_no_est_disp}}\hfill
	\caption{FSI sub-iterations for the test cases with and without the prediction of the displacements.}
	\label{fig:used_iterout_comparison}
\end{figure}
\begin{figure}[H]
	\centering
	\subfigure[Simulation with estimation of displacement.]{\includegraphics[width=0.495\textwidth]{\FigPath/Masterarbeit/res_disp_convergence_itout20_est_disp.pdf} \label{fig:residuum_convergence_est_disp}}\hfill
	\subfigure[Simulation without estimation of displacement.]{\includegraphics[width=0.495\textwidth]{\FigPath/Masterarbeit/res_disp_convergence_itout20_no_est_disp.pdf}\label{fig:residuum_convergence_no_est_disp}}\hfill
	\caption{Achievement of the FSI convergence criterion $\epsilon_{FSI,\,disp}<1{\cdot}10^{-6}$ for the test cases with and without estimation of the displacements.}
	\label{fig:residuum_convergence_comparison}
\end{figure}
\par Furthermore, since the Fig.\ \ref{fig:residuum_convergence_comparison} does not show in detail the residuum of displacement at each sub-iteration, this is meticulously illustrated in Fig.\ \ref{fig:residuum_comparison} for the last five time steps of each simulation. These once again indicate that although all twenty sub-iterations are computed, the FSI convergence criterion is not achieved for the simulations without the estimation of displacements, resulting in a lost of accuracy.
\begin{figure}[H]
	\centering
	\subfigure[Simulation with estimation of displacement (\mbox{$9{,}996\leq n\leq10{,}000$}).]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/res_disp_itout20_est_disp.pdf} \label{fig:residuum_est_disp}}\hfill
	\subfigure[Simulation without estimation of displacement (\mbox{$14{,}282\leq n\leq14{,}286$}).]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/res_disp_itout20_no_est_disp.pdf}\label{fig:residuum_no_est_disp}}\hfill
	\caption{Residuum of displacement and force in the $x_3$-direction at the last five time steps of the simulations with and without estimation of displacement.}
	\label{fig:residuum_comparison}
\end{figure}
\par The accuracy of both methods can be analyzed according to the lift forces $F_3$, which should not be produced since the symmetric NACA0012 airfoil is at an incidence of $\alpha=0^\circ$. Table \ref{table:comp_forces_est_disp} illustrates the time-averaged lift force for the cases with and without estimation of displacement. 
\begin{table}[H]
	\centering
	\begin{tabular}{p{3cm} p{3cm} p{5cm}}
		\hline
		\multirow{2}{3cm}{\centering{\bf{Estimation of displacement}}} &  \multicolumn{2}{c}{\bf{Time-averaged lift force ($\text{kg}{\cdot}\text{m}{\cdot}\text{s}^{-1})$}} \tabularnewline \cline{2-3}
		& \centering{\bf{Mean}} & \centering{\bf{Standard deviation}} \tabularnewline\hline
		\centering{Yes} & \centering{$3.343{\cdot}10^{-7}$}&\centering{$4.341{\cdot}10^{-7}$} \tabularnewline
		\centering{No} & \centering{$1.306{\cdot}10^{-7}$}&\centering{$6.226{\cdot}10^{-6}$} \tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:comp_forces_est_disp}Time-averaged lift forces of the cases with and without the prediction of the displacements.}
\end{table}
\par Although the mean value of the time-averaged lift forces is slightly higher for the case utilizing the estimation of displacement, the standard deviation is one order of magnitude lower. Then, the calculations that utilize this prediction present a smaller dispersion of the data, as shown in Fig.\ \ref{fig:lift_comparison}. Therefore, the forces at each time step tend to be closer to the mean value. Hence, the algorithm that predicts the displacements leads to a greater accuracy.
\par Finally, the simulation of the fluid-structure interaction with the prediction of the displacements is also approximately $6.7$ times faster, since it requires the computation of less sub-iterations in order to converge. Thus, the estimation of displacements is applied for all simulations in order to enable a faster convergence of the FSI solution and consequently save computational time.
\begin{figure}[H]
	\centering
	\subfigure[Simulation with estimation of displacement.]{\includegraphics[width=0.495\textwidth]{\FigPath/Masterarbeit/force_y_itout20_est_disp.pdf} \label{fig:lift_est_disp}}\hfill
	\subfigure[Simulation without estimation of displacement.]{\includegraphics[width=0.495\textwidth]{\FigPath/Masterarbeit/force_y_itout20_no_est_disp.pdf}\label{fig:lift_no_est_disp}}\hfill
	\caption{Lift forces for the test cases with and without the prediction of the displacements.}
	\label{fig:lift_comparison}
\end{figure}


\subsection{Investigation of the added mass effect}
\label{subsec:added_mass_effect}
\par Added mass is the additional inertia added to a system composed of a fluid and a body, which is submitted to a relative velocity. The deflection of the fluid due to the presence of the body generates additional fluid forces, which act on the surfaces in contact with the flow. This added mass acts as an extra mass on the structural degrees of freedom at the coupling interface and has destabilizing effects on loose coupled algorithms due to their explicit nature. Moreover, the effect of this mass varies also with the time discretization methods utilized by the structural and fluid subproblems (see \mbox{Förster et al.\ \cite{Foerster_2007})}.
\par The relation between the mass of the body and the mass of the displaced fluid \mbox{(see Eq.\ \ref{eq:mass_ratio})} indicates if the added mass effect must be considered.  The higher this relation, the smaller the effect of the added mass and therefore sequentially staggered schemes (loose coupling) are numerically stable and can be utilized (see Causin et al.\ \cite{Causin_2005}).
\begin{equation}
\label{eq:mass_ratio}
m^*=\frac{m^{body}}{m^{fluid}_{disp}}
\end{equation}
\par Song et al.\ \cite{Song_2013} investigated the influence of the added mass effect on stiff plate structures of different materials utilizing a partitioned approach based on a loose coupling algorithm. The case with $m^*=10$ exhibited no convergence problems, while under-relaxation factors were used in the case with $m^*=1$ in order to guarantee the convergence of the solution. Therefore, the influence of the added mass effect for $m^*=10$ was negligible, while this effect was responsible for numerical difficulties for the $m^*=1$ case.  
\par In the present work, the mass ratio between airfoil and displaced fluid is $m^*=720$. Therefore, a loose coupling method ($n_{FSI}=1$) can be utilized due to its numerical stability and lower required computational time (compared to strong coupling approaches). 


\subsection{Investigation of the coupling algorithm}
\label{subsec:investigation_coupling_algorithm}

\par Although the added mass effect is negligible for the NACA0012 FSI test cases (see Section \ref{subsec:added_mass_effect}), the accuracy of the loose coupling algorithm is tested through a comparison between the airfoil responses computed with both explicit and implicit coupling approaches. Three simulations with two degrees of freedom (pitch and plunge) are performed with the $m{-}L_3^{min}{-}y_{max}^+$ mesh, the mapping strategy 4 (see Section \ref{subsubsec:study_mapping_strategy}), the TFI re-meshing method and the prediction of displacements until a dimensionless time of $t^*=1564.5$ is achieved. The simulated Reynolds number is $Re=30{,}000$ and the utilized linear and torsional stiffnesses are  $k_{l,\,2}=144\,\text{N}{\cdot}\text{m}^{-1}$ and $k_{t,\,3}=0.3832\text{N}\,\text{m}{\cdot}\text{rad}^{-1}$, respectively.
\par The properties of the simulations are summarized in Table \ref{table:comp_FSI_coupling}, regarding that a test case that solves the fluid domain with an implicit coupling algorithm for the first \mbox{$n=100{,}000$} times steps and afterwards with an explicit algorithm is also computed.
\begin{table}[H]
	\centering
	\begin{tabular}{p{2.8cm} p{4.1cm} p{2.0cm} p{3cm} p{1.8cm}}
		\hline
		\multicolumn{1}{c}{\multirow{3}{*}{\centering{\bf{Mesh}}}} & \multicolumn{1}{c}{\multirow{3}{*}{\centering{\bf{Coupling algorithm}}}} & \centering{\bf{Maximal iteration number}} & \centering{\bf{Maximal number of FSI sub-iterations}} & \centering{\bf{Time step size (s)}}\tabularnewline \hline
		\centering{$m{-}L_3^{min}-y^{+}_{max}$} & \centering{Loose} & \centering{$3{,}500{,}000$} & \centering{1} & \centering{$1\cdot10^{-5}$} \tabularnewline \hline
		\centering{$m{-}L_3^{min}{-}y^+_{max}$} & \centering{Strong} & \centering{$3{,}500{,}000$} &\centering{20} & \centering{$1\cdot10^{-5}$} \tabularnewline \hline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{$m{-}L_3^{min}{-}y^+_{max}$}}} & \centering{Strong for $n\leq100{,}000$} & \centering{$100{,}000$} & \multicolumn{1}{c}{\centering{20}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{$1\cdot10^{-5}$}}} \tabularnewline	\cline{2-4}
		& \centering{Loose for $n>100{,}000$} & \centering{$3{,}500{,}000$} & \centering{1} & \tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:comp_FSI_coupling}Simulation properties of the test cases aimed at the comparison of the coupling algorithms.}
\end{table}
\par The maximal number of sub-iterations is set to $n_{FSI}=20$ for the cases with strong coupling, since this is sufficient and necessary to achieve the convergence criterion of all computed time steps, especially during the initialization phase. After this phase, however, only two sub-iterations are in general utilized by the FSI solver (see Section \ref{subsec:investigation_estimation_displacement}), due to the fact that the convergence criterion is achieved before all sub-iterations are performed.
\par The airfoil structural responses in the form of translational displacements in the \mbox{$x_2$-direction} and rotational displacements about the $x_3$-axis are illustrated in Fig.\ \ref{fig:displacements_coupling_investigation} as a function of the time. Since the fluid movement is chaotic, a direct comparison of the displacements achieved by the different coupling algorithms is not possible. Therefore, only the oscillation amplitudes are studied and compared.
\par All simulated coupling algorithms are characterized by the achievement of the same maximal amplitude of oscillation, regarding the plunge and pitch degrees of freedom. For instance, these values are \mbox{$X_2=1.8{\cdot}10^{-4}\,\text{m}$} and \mbox{$\varphi_3=0.33^\circ$} for the translational and rotational motions, respectively. Although the various coupling algorithms require different initialization times in order to achieve a limit-cycle oscillation, the amplitudes of these oscillations are also the same for all coupling approaches, that is, \mbox{$X_{2,\,LCO}=1.8{\cdot}10^{-4}\,\text{m}$} and \mbox{$\varphi_{3,\,LCO}=0.0135^\circ$}.
\begin{figure}[H]
	\centering
	\subfigure[Loose coupling algorithm: Translational displacement $X_2$.]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/trans_disp_kl_144_tfi_loose.pdf} \label{fig:frequenciess_translation}}\hfill
	\subfigure[Loose coupling algorithm: Rotational displacement $\varphi_3$.]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/rot_disp_kl_144_tfi_loose.pdf}\label{fig:frequencies_rsotation}}\hfill
	\centering
	\subfigure[Strong coupling algorithm for $t\leq1\,s$ and loose coupling algorithm for $t>1\,s$: Translational displacement $X_2$.]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/trans_disp_kl_144_tfi_start_loose.pdf} \label{fig:frequencies_translatison}}\hfill
	\subfigure[Strong coupling algorithm for $t\leq1\,s$ and loose coupling algorithm for $t>1\,s$: Rotational displacement $\varphi_3$.]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/rot_disp_kl_144_tfi_start_loose.pdf} \label{fig:frequencies_translatiosn}}\hfill
%\end{figure}
%\begin{figure}[H]
	\subfigure[Strong coupling algorithm: Translational displacement $X_2$.]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/trans_disp_kl_144_tfi_strong.pdf} \label{fig:frequencies_translatsiosn}}\hfill
	\subfigure[Strong coupling algorithm: Rotational displacement $\varphi_3$.]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/rot_disp_kl_144_tfi_strong.pdf} \label{fig:frequencies_stranslation}}\hfill
	\caption{Comparison of the coupling algorithms: Translational ($X_2$) and rotational ($\varphi_3$) displacements.}
	\label{fig:displacements_coupling_investigation}
\end{figure}
\par Since the amplitudes achieved with the loose coupling algorithm are in a good agreement with the ones achieved with both other simulated test cases, this coupling does not influence the computation of the fluid domain and therefore is applicable to further simulate the fluid structure interaction between the NACA0012 airfoil and the flow. This result is expected, since this FSI is characterized by a negligible added mass effect (see \mbox{Section \ref{subsec:added_mass_effect}).} Nevertheless, the frequencies generated by the fluid-structure interaction are also investigated.
\par In order to analyze the frequency domain, a Fourier transform with a Hamming window is carried out, considering that the independent variable is the time $t$ and that the dependent variables are the plunge and pitch displacements, i$.$e$.$, respectively $X_2$ and $\varphi_3$. The latter are utilized as parameters for the Fourier transform since these generate more distinct peaks in the frequency domain, when compared to the lift and drag forces, facilitating the comparison of the coupling algorithms. The frequency domain of the translational and rotational displacements are illustrated in Fig.\ \ref{fig:frequencies_displacements_coupling}, regarding that the amplitudes are normalized in relation to the maximal value. The frequency domain of the simulation characterized by the utilization of both loose and strong coupling algorithms is not displayed since only unclear frequency peaks are formed due to the fact that this test case requires a longer initialization time and therefore not enough data regarding the fully developed state is available. 
\begin{figure}[H]
	\centering
	\subfigure[Loose coupling.]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/frequencies_X2_phi3_loose_max_normalized.pdf} \label{fig:frequencies_loose}}\hfill
	\subfigure[Strong coupling. BLABLA]{\includegraphics[width=0.48\textwidth]{\FigPath/Masterarbeit/frequencies_X2_phi3_strong_max_normalized.pdf}\label{fig:frequencies_strong}}\hfill
	\caption{Frequency domain of the plunge ($X_2$) and pitch ($\varphi_3$) displacements.}
	\label{fig:frequencies_displacements_coupling}
\end{figure}
\par The frequencies of the three peaks characterized by the highest amplitudes are described in \mbox{Table \ref{table:frequencies_coupling}} for both strong and loose coupling algorithms. The origin of the generated frequencies and their physical or numerical meaning are not investigated, since these test cases aim only at the comparison of the coupling algorithms. Since only minor deviations are present in the frequencies generated by both coupling algorithms, it is confirmed that the coupling method does not influence the calculation of the coupled problem. 
\begin{table}[H]
	\centering
	\begin{tabular}{p{2cm} p{3cm} p{3cm} p{3cm}}
		\hline
		\centering{\bf{FSI coupling}} & \centering{\bf{Frequency $f_1$ ($\text{Hz}$)}} & \centering{\bf{Frequency $f_2$ ($\text{Hz}$)}} &  \centering{\bf{Frequency $f_3$ ($\text{Hz}$)}} \tabularnewline \hline
		\centering{Strong} & \centering{2.886} & \centering{5.772} & \centering{8.658} \tabularnewline
		\centering{Loose} & \centering{2.859} & \centering{5.719} & \centering{8.580} \tabularnewline		
		\hline	
	\end{tabular}
	\caption{\label{table:frequencies_coupling}Characteristic frequencies: Simulations with different coupling schemes.}
\end{table}
\par Finally, the computational time of all simulations are compared, according to \mbox{Table \ref{table:compt_time_coupling}}. The loose coupling algorithm requires about $85\%$ and $56\%$ of the computational time of respectively the test case characterized by the utilization of both couplings and the one applying solely the loose coupling algorithm. Since it is also proven that the explicit coupling is accurate, this is utilized for the further investigations of the fluid-structure interaction.
\begin{table}[H]
	\centering
	\begin{tabular}{p{4.2cm} p{5cm}}
		\hline
		\centering{\bf{FSI coupling}} & \centering{\bf{Computational time (d)}} \tabularnewline \hline
		\centering{Loose} &  \centering{23.07} \tabularnewline	
		\centering{Strong for $n\leq100{,}000$} & \multicolumn{1}{c}{\multirow{2}{*}{{$27.05$}}} \tabularnewline	
		\centering{Loose for $n>100{,}000$} & \tabularnewline
		\centering{Strong} & \centering{$41.23$} \tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:compt_time_coupling}Computational times: Simulations with different coupling schemes.}
\end{table}

\subsection{Conclusions}
\label{conclusions_FSI_coupling}

\par The thorough analysis of the implemented estimation of displacements algorithm points out that this prediction improves the convergence properties of coupled problems while maintaining the accuracy. For the NACA0012 FSI test cases, the application of this estimation reduced $85\%$ of the computational time, when comparing to a computation that does not utilize this algorithm.
\par The investigation of the mass ratio proves that the added mass effect is negligible. Therefore, the FSI computation is not characterized by convergence problems, i$.$e$.$, even the explicit coupling is stable. Due to the fact that the loose coupling scheme requires only $56\%$ of the time required by the strong coupling algorithm, this explicit coupling together with the prediction of the displacements is further applied in the FSI test cases.


==> 4.tex <==
\chapter{Free rigid NACA0012 airfoil in turbulent flows: Geometry and setup}
\label{chap:FSI_flow_NACA0012}

\par The NACA0012 airfoil is a symmetric profile usually utilized for stability purposes in airplanes, such as in horizontal and vertical stabilizers. Therefore, it is commonly investigated by numerical and experimental studies and thus a vast literature is available, enabling the establishment of the model ability to reproduce the physics, i$.$e$.$, the model validation.
\par The current work is a continuation of the NACA0012 airfoil investigations performed by Streher \cite{Streher_2017}, which were aimed at the investigation of the flow characteristics for a fixed airfoil at different angles of attack and submitted to a Reynolds number of $Re=100{,}000$. The wall-resolved LES simulations utilizing the Smagorinsky model were validated through a comparison with numerical and experimental results available in the literature. The present work, then, expands this model in order to perform fluid-structure interaction simulations.

\section{Test section geometry}\markboth{CHAPTER 2.$\quad$FREE RIG. NACA0012 AIR. IN TURB. FLOWS}{2.1$\quad$TEST SEC. GEO.}
\label{sec:geometry}
\par The NACA0012 profile stands for the National Advisory Committee for Aeronautics four digit series airfoil profiles. The first two digits, i.e$.$, $00$, represent a symmetrical airfoil and the last two stand for a profile with a maximal thickness of twelve percent of the chord length $c$, located at thirty percent of the chord \cite{Jacobs_1935}. 
\par The modeled airfoil has a chord length of $c=0.1\,m$ and a sharp trailing edge. This is described by NASA \cite{NASA_2016} through Eq.\ (\ref{eq:NACA0012}). The origin of the global coordinate system is located at the leading edge. $X_{N,\,2}$ and $X_{N,\,1}$ represent the vertical and horizontal coordinates of the airfoil, respectively. 
\begin{eqnarray}
\nonumber
\label{eq:NACA0012}
X_{N,\,2}&=&\pm 0.59468918c\left[0.29822277\sqrt{\frac{X_{N,\,1}}{c}}-0.12712523\frac{X_{N,\,1}}{c}-0.35790791\left(\frac{X_{N,\,1}}{c}\right)^2\right.\\
&&+0.29198497\left(\frac{X_{N,\,1}}{c}\right)^3\left.-0.10517461\left(\frac{X_{N,\,1}}{c}\right)^4\right]
\end{eqnarray}
\par The two-dimensional geometry of the computational fluid domain is established with help of artificial boundaries, which are carefully chosen according to the work of Almutari \cite{Almutari_2010}. This presents the results of various wall-resolved large-eddy simulations for a fixed rigid NACA0012 profile at diverse configurations of Reynolds numbers and angles of attack, which are validated by a-posteriori studies against the results of DNS simulations achieved by \mbox{Jones et al. \cite{Jones_2008}}, as well as by the experimental results of Rinoiei and Takemura \cite{Takemura_2004}. Moreover, this test section geometry is already tested with the in-house software FASTEST-3D for the case of wall-resolved LES of a fixed rigid NACA0012 at a Reynolds number of $Re=100{,}000$ (see Streher \cite{Streher_2017}), delivering satisfactory results.
\par Figure \ref{fig:fluid_domain_3d} illustrates the simulated fluid domain and the curvilinear coordinates $\eta$ and $\xi$ utilized in order to simplify the description of the meshes. The test section is characterized by the wake length $W=5\,c$ and the domain radius $R=7.3\,c$. Due to a contradiction between the span-wise lengths suggested by Almutari \cite{Almutari_2010} and by Schmidt \cite{Schmidt_2016}, i$.$e$.$, respectively $L_3=0.5\,c$ and \mbox{$L_3=0.25\,c$}, the influence of this parameter is investigated and discussed in Section \ref{sec:study_span_wise_length}. Since the best compromise between accuracy and computational time is achieved for the narrowest geometry, i$.$e$.$, $L_3=0.25\,c$, this is utilized for the further investigations. 
\begin{figure}[H]
	\centering
	\centering
	\includegraphics[scale=0.85,draft=\drafttype]{\FigPath/Masterarbeit/Koordinaten_System.pdf}
	\caption{\label{fig:fluid_domain_3d}Fluid domain of the NACA0012 airfoil profile.}
\end{figure}

\section{Computational meshes}\markboth{CHAPTER 2.$\quad$FREE RIG. NACA0012 IN TURB. FLOWS}{2.2$\quad$COMPT. MESHES}
\label{sec:meshes}
\par The computational fluid domain is discretized into several control volumes by the software ANSYS ICEM CFD. Three different C block-structured hexahedral grids with varying number of nodes $N$ and first cell heights $\Delta y^{\,first\;cell}$ are generated. \mbox{Table \ref{table:mesh_parametes}} indicates the different grid parameters. Figure \ref{fig:coarse_grid} illustrates the $m{-}L_3^{min}{-}y^{+}_{max}$ grid, regarding that only one out of two mesh lines is delineated in the $\xi$ and the $\eta$ axes in order to achieve a good quality image.
\par $N_W$, $N_R$, $N_{L_3}$ and $N_{SS}$ represent the number of nodes utilized to discretize the edges of the wake, domain radius, span-wise length and suction side of the airfoil, respectively. Since the NACA0012 airfoil is symmetric, a equal number of nodes is applied at the pressure and suction side edges.
\par The generated meshes are composed of twelve geometrical blocks characterized by smooth transitions on the interfaces. The stretching factor of the wake and domain radius edges are respectively $q_W=1.07$ and $q_R=1.1$. The mesh quality is evaluated according to the determinant of the Jacobi-Matrix and the internal angles of every control volume, regarding that target values of respectively $1$ and $90^\circ$ are aimed at in order to accomplish a mesh composed of only orthogonal cells with a perfect shape. Since all cells of the generated grids have determinants of the Jacobi-Matrix greater than $0.85$ and internal angles greater than $81^\circ$, these are considered high-quality meshes.
\begin{table}[H]
	\centering
	\begin{tabular}{p{2.5cm} p{2.3cm} p{3.5cm} p{1.7cm} p{0.5cm} p{0.5cm} p{0.5cm} p{0.5cm}}
		\hline
		\multicolumn{1}{c}{\multirow{2}{*}{\centering{\bf{Mesh}}}} & \centering{\bf{Span-wise length $L_3$}} & \centering{\bf{First cell heigth $\Delta y^{\,first\;cell}$ (m)}} & \centering{\bf{Control volumes}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{\bf{$N_W$}}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{\bf{$N_R$}}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{\bf{$N_{L_3}$}}}} & \multicolumn{1}{c}{\multirow{2}{*}{\centering{\bf{$N_{SS}$}}}} \tabularnewline 
		\hline
		\centering{$m{-}L_3^{min}{-}y^{+}_{min}$} & \centering{0.25\,c}& \centering{$1.8\cdot10^{-6}$} & \centering{1{,}065{,}600} & \centering{91} & \centering{61} & \centering{61} & \centering{63} \tabularnewline
		\centering{$m{-}L_3^{min}{-}y^{+}_{max}$} & \centering{0.25\,c}& \centering{$5.0\cdot10^{-6}$} & \centering{1{,}065{,}600} & \centering{91} & \centering{61} & \centering{61} & \centering{63} \tabularnewline
		\centering{$m{-}L_3^{max}{-}y^{+}_{min}$} & \centering{0.50\,c}& \centering{$1.8\cdot10^{-6}$} & \centering{2{,}131{,}200} & \centering{91} & \centering{61} & \centering{121} & \centering{63} \tabularnewline
		\hline
	\end{tabular}
	\caption{\label{table:mesh_parametes}Parameters applied for the grid generation.}
\end{table}
\begin{figure}[H]
	\centering
	\subfigure[Overall view.]{\includegraphics[width=0.495\textwidth]{\FigPath/Masterarbeit/grob_grid_5e-5_wall_distance_lz_0pt25.pdf}\label{fig:mesh}}\hfill
	\subfigure[Mesh near the airfoil.]{\includegraphics[width=0.495\textwidth]{\FigPath/Masterarbeit/grob_grid_5e-5_wall_distance_lz_0pt25_zoom.pdf} \label{fig:mesh_zoom}}\hfill
	\caption{$m{-}L_3^{min}{-}y^{+}_{max}$ mesh.}
	\label{fig:coarse_grid}
\end{figure}  
\par Mesh independence studies are carried out for all three grids in \mbox{Appendix \ref{sec:study_span_wise_length} and \ref{sec:investigation_first_cell_height}}. These are based on the analysis of the aerodynamic coefficients, as well as  of the dimensionless wall distance. They assure that even the $m{-}L_3^{min}{-}y^{+}_{max}$ mesh, which requires the smallest computational effort, does not affect the results. Therefore, the $m{-}L_3^{min}{-}y^{+}_{max}$ grid is further applied for the FSI test cases.

\section{CFD setup}\markboth{CHAPTER 2.$\quad$FSI BETWEEN FLOW AND NACA0012 AIR.}{2.3$\quad$CFD SETUP}
\label{sec:CFD_setup}
\par The numerical methodologies described in Section \ref{sec:CFD} are applied in conjunction with the following CFD setup in order to solve the computational domain. The fluid and simulation parameters are summarized in Tables \ref{table:flow_parameters} and \ref{table:simulation_parameters}. The temperature is presumed to be constant and the fluid incompressible. The inflow velocities in the $x_2$ and $x_3$ directions are assumed to be $u_{in,\,2}=u_{in,\,3}=0\,m{\cdot}s^{-1}$. The Reynolds number is calculated using the free-stream conditions and the airfoil chord length, i$.$e$.$, $c=0.1\,m$.
\par Although Streher \cite{Streher_2017} applied a Reynolds number of $Re=100{,}000$ in the wall-resolved simulations of a fixed rigid NACA0012 airfoil, this work approximates the computational domain of the same airfoil at a Reynolds number of $Re=30{,}000$ in order to acquire less computational intensive simulations. This reduction of the Reynolds number allows the computation of the fluid structure interaction with a coarser grid, i$.$e$.$, $m{-}L_3^{min}{-}y^{+}_{max}$, which is composed of about $14\%$ of the nodes of the coarser grid applied by \mbox{Streher \cite{Streher_2017}}. Moreover, the height of the cells located on the airfoil surface are approximately triplicated while the time step size is increased in approximately two orders of magnitude. Therefore, the required computational time is reduced in $95.5\%$.
\begin{table}[!htbp]
	\centering
	\begin{tabular}{l l}
		\hline
		Temperature & $T=300\,\text{K}$ \tabularnewline 
		Inflow velocity & $u_{in,\,in}=4.47\;\text{m}{\cdot}\text{s}^{-1}$ \tabularnewline
		Fluid density & $\rho_f=1.225\;\text{kg}{\cdot}\text{m}^{-3}$ \tabularnewline
		Dynamic fluid viscosity & $\displaystyle{\mu_f=18.27\cdot10^{-6}\;\text{Pa}{\cdot}\text{s}}$ \tabularnewline
		Reynolds number & $\displaystyle{Re=\frac{u_{in,\,1}\;\rho_f\;c}{\mu_f}=30{,}000}$ \tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:flow_parameters}Fluid parameters.}
\end{table}
\begin{table}[!htbp]
	\centering
	\begin{tabular}{l l}
		\hline
		Spatial discretization & FVM \tabularnewline
		Temporal discretization & Predictor-corrector scheme \tabularnewline
		Turbulence approach & LES \tabularnewline
		Sub-grid scale model & Smagorinsky \tabularnewline
		Damping function & Van-Driest \tabularnewline
		Smagorinsky constant & $C_s=0.1$ \tabularnewline 
		Wall function & None \tabularnewline
		\multirow{2}{*}{Mesh adaption} & Small displacements: TFI \tabularnewline
		& Large displacements: Hybrid IDW-TFI\tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:simulation_parameters}Simulation parameters.}
\end{table}

\subsection{Initial conditions}
\label{sec:CFD_initial_conditions}
\par The conservation laws are parabolic in time. Therefore, initial conditions for the whole fluid domain are required. In the current work, these conditions are applied for the velocity vector and pressure in relation to a Reynolds number of $Re=30{,}000$, according to \mbox{Eqs.\ (\ref{eq:initial_velocity_i})} through (\ref{eq:initial_pressure}). The initial velocity vector is characterized only by a velocity in the main flow direction (chord-wise direction), which is equal to the inlet velocity vector (see \mbox{Section \ref{subsubsec:inflow}}).
\begin{eqnarray}
u_{t_0,\,1}&=&4.47\;\text{m}{\cdot}\text{s}^{-1} \label{eq:initial_velocity_i}\\
u_{t_0,\,2}&=&0\;\text{m}{\cdot}\text{s}^{-1} \label{eq:initial_velocity_j}\\
u_{t_0,\,3}&=&0\;\text{m}{\cdot}\text{s}^{-1} \label{eq:initial_velocity_k}\\
p_{t_0}&=&0\;Pa \label{eq:initial_pressure}
\end{eqnarray}

\subsection{Boundary conditions}
\label{sec:CFD_boundary_conditions}
\par The incompressible governing equations are elliptical in space. Therefore, the definition of boundary conditions for all boundaries is mandatory.

\subsubsection{Inlet}
\label{subsubsec:inflow}
\par The inlet velocity tensor, i$.$e$.$, velocity vector of the cells located at the inlet boundary, is given in the Dirichlet form and is illustrated in \mbox{Eqs.\ (\ref{eq:inlet_velocity_1})} through (\ref{eq:inlet_velocity_3}) for a Reynolds number of $Re=30{,}000$:
\begin{eqnarray}
u_{in,\,1}&=&4.47\;\text{m}{\cdot}\text{s}^{-1} \label{eq:inlet_velocity_1}, \\
u_{in,\,2}&=&0\;\text{m}{\cdot}\text{s}^{-1} \label{eq:inlet_velocity_2}, \\
u_{in,\,3}&=&0\;\text{m}{\cdot}\text{s}^{-1} \label{eq:inlet_velocity_3}. \\
\end{eqnarray}
\par A pressure boundary condition (Eq. (\ref{eq:inlet_pressure})) in the Neumann form is utilized for the pressure correction $p^{\,corr}$, according to the work of Münsch \cite{Muensch_2015}:
\begin{equation}
\left. \frac{\quad \partial p^{\,corr}}{\partial x_1}\right |_{in}=0.
\label{eq:inlet_pressure}
\end{equation}

\subsubsection{Symmetry boundary}
\label{subsubsec:symmetry_boundary_condition}
\par A symmetry boundary can be used if both geometry and flow behavior have mirror symmetry, which is never the case of turbulent flows. However, since the edges located at the top and the bottom of the fluid domain are situated sufficiently far from the airfoil wake, these can be approximated as symmetric. These edges are characterized by zero velocities normal to the boundary, according to Eqs.\ (\ref{eq:symmetry_1}) through (\ref{eq:symmetry_3}): 
\begin{eqnarray}
u_{sym,\,1}&\neq&0\;\text{m}{\cdot}\text{s}^{-1}, \label{eq:symmetry_1} \\ 
u_{sym,\,2}&=&0\;\text{m}{\cdot}\text{s}^{-1}, \label{eq:symmetry_2} \\ 
u_{sym,\,3}&\neq&0\;\text{m}{\cdot}\text{s}^{-1}. \label{eq:symmetry_3}
\end{eqnarray}
\par Furthermore, only a velocity gradient of $u_2$ in relation to the $x_2$ direction is available (see Münsch \cite{Muensch_2015}). Therefore, only the shear stress component $\tau_{22}$ is present in the symmetry edges, conform Eqs.\ (\ref{eq:symmetry_flux_1}) through (\ref{eq:symmetry_flux_3}):
\begin{eqnarray}
\tau_{sym,\,12}&=&-\;\;\mu\left.\frac{\partial u_1}{\partial x_2}\right|_{sym}=0, \label{eq:symmetry_flux_1} \\ 
\tau_{sym,\,22}&=&-2\mu\left.\frac{\partial u_2}{\partial x_2}\right|_{sym}\neq0, \label{eq:symmetry_flux_2} \\ 
\tau_{sym,\,32}&=&-\;\;\mu\left.\frac{\partial u_3}{\partial x_2}\right|_{sym}=0. \label{eq:symmetry_flux_3}
\end{eqnarray}

\subsubsection{No-slip wall}
\label{subsubsec:wall}
\par The no-slip wall condition states that a fluid adheres to the wall and consequently moves with its velocity. For the case of fluid-structure interaction, a boundary condition in the form of Dirichlet is applied. This indicates that the flow velocity at the moving wall $u_{w,\,i}$ is equal to the body velocity $u_{body,\,i}$, as stated in Eq.\ (\ref{eq:wall_velocity}):
\begin{equation}
\label{eq:wall_velocity}
u_{w,\,i}=u_{body,\,i}.
\end{equation}
\par The structure velocity is approximated according to a first order accuracy difference approximation scheme. This is based on the time step size $\Delta t$, as well as on the structural displacements $X_i$ at the last time step $n$ and at the current time step $n+1$ \mbox{(see Münsch \cite{Muensch_2015})}:
\begin{equation}
\label{eq:body_velocity}
u_{body,\,i}^{n+1}=\frac{X_i^{n+1}-X_i^n}{\Delta t}.
\end{equation}
\par The no-slip wall also states a boundary condition in the form of Neumann for the pressure, according to Eq.\ (\ref{eq:wall_pressure}):
\begin{equation}
\left.\frac{\partial p}{\partial \eta}\right |_w=0. \label{eq:wall_pressure}
\end{equation}

\subsubsection{Outlet}
\label{subsubsec:outlet}
\par The outlet boundary must be located where the eddies can pass through at most undisturbed and without reflection, so that this edge has no or only a minor influence on the domain, as described by Breuer \cite{Breuer_2013}. 
\par The FSI simulation of the NACA0012 profile requires the usage of a transport equation, i.e$.$, a convective equation, for the outlet boundary:
\begin{equation}
\label{eq:outlet_boundary}
\frac{\partial u_i}{\partial t}+U_{conv}\left.\frac{\partial u_i}{\partial x_1}\right|_{out}=0.
\end{equation}
\par The convective velocity $U_{conv}$ is parallel to the stream-wise direction and therefore normal to the outlet boundary. In the present case $U_{conv}$ is set to the free stream velocity, i.e$.$, $U_{conv}=u_{in,\,1}=4.47\,m{\cdot}s^{-1}$.
\par Due to the extrapolation of the velocities on the outlet boundary, a zero gradient of the pressure correction is available (see Eq.\ (\ref{eq:outlet_pressure})), as stated by Münsch \cite{Muensch_2015}. 
\begin{equation}
\left.\frac{\quad \partial p^{\,corr}}{\partial x_1}\right |_{out}=0 \label{eq:outlet_pressure}
\end{equation}


\subsubsection{Periodic boundary}
\label{subsubsec:periodic_boundary_condition}
\par The periodic boundary condition allows the reduction of the fluid domain and consequently the decrease of the computational effort. It is based on the simultaneous usage of the boundary values on two correspondent domain boundaries, as stated by Breuer \cite{Breuer_2002}.
\par The usage of this type of boundary is, however, only possible in homogeneous directions, which are characterized by the non-variation of the statistical flow. The period length must be carefully chosen in order to guarantee the capture of the largest eddies. This can be assured through the calculation of the turbulent fluctuation two-point correlation, which must tend to zero (see Breuer \cite{Breuer_2002}).
\par In the case of the FSI investigations of the NACA0012 airfoil, the span-wise direction is homogeneous and characterized by \mbox{$u_i(x_1,x_2,x_3,t)=u_i(x_1,x_2,x_3+\Delta x_3,t)$} and \mbox{$p(x_1,x_2,x_3,t)=p(x_1,x_2,x_3+\Delta x_3,t)$.} A periodic boundary condition is, then, applied in this direction. Two period lengths of $L_3=0.5\,c$ and $L_3=0.25\,c$ are tested and thoroughly discussed in Appendix \ref{sec:study_span_wise_length}. Since the best compromise between accuracy and computational time is achieved with $L_3=0.25\,c$, this is applied for the computation of the FSI test cases.

\section{CSD setup}
\label{sec:CSD_setup}
\par The CSD setup is configured according to the rigid NACA0012 model utilized by the experimental setup, which is thoroughly discussed in Appendix \ref{appendix_experimental_setup}. The structural properties, as well as the initial and boundary conditions are set in the $csdvalues.dat$ file, which is compiled by the rigid movement solver during the initialization sub-routine. This file is described in Table \ref{table:csdvalues} for the FSI cases with plunge and pitch degrees of freedom, i$.$e$.$, translational degree of freedom in the $x_2$-direction and rotational degree of freedom about the $x_3$-axis ($\varphi_3$), respectively..
\par Boolean algebra is utilized in order to define the system degrees of freedom (DOF): the first three inputs are regarding the three translational degrees of freedom in the $x_1$, $x_2$ and $x_3$ directions, while the last three stand for the rotations about the $x_1$, $x_2$ and $x_3$ axes ($\varphi_1$, $\varphi_2$ and $\varphi_3$, respectively). If a degree of freedom is not considered \mbox{(set to false $F$)}, all variables of this column, with an exception of the mass moment of inertia, are set to zero by the initialization subroutine. 
\par The initial conditions are given in the form of initial displacements, velocities and accelerations, while the boundary conditions are given by the external (fluid) forces and moments computed by the CFD solver. Since the body is initially in dynamic equilibrium, all this conditions are zero at $t=0\,s$.
\par The body properties are given by the mass and the mass moment of inertia tensor, according to lines five and nine of the initialization file. The spring stiffness and the damping ratio (see Eq.\ (\ref{eq:damping_ratio})) are given in the sixth and seventh lines, respectively. The location of the body-fixed undeformed Cartesian coordinate system in relation to origin of the Cartesian coordinate system established by the CFD mesh (global CCS), is given by the last line of the $csdvalues.dat$ file. In order to guarantee an uncoupled system, the body-fixed undeformed Cartesian coordinate system is located at the airfoil center of mass (see Section \ref{subsec:moment_inertia}).
\begin{table}[H]
	\centering
	\begin{tabular}{p{2.8cm} | p{1.7cm} p{1.7cm} p{1.7cm} p{1.7cm} p{1.7cm} p{1.7cm}}
		\cline{1-7}
		\centering{\bf{$\,$}}  & \centering{\bf{$x_1$}} & \centering{\bf{$x_2$}} & \centering{\bf{$x_3$}} & \centering{\bf{$\varphi_1$}} & \centering{\bf{$\varphi_2$}} & \centering{\bf{$\varphi_3$}} \tabularnewline \hline
		\centering{\bf{DOF}} & \centering{F} &\centering{T} & \centering{F} & \centering{F} & \centering{F} & \centering{T} \tabularnewline
		\centering{\bf{Displacement}} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} \tabularnewline
		\centering{\bf{Velocity}} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} \tabularnewline
		\centering{\bf{Acceleration}} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} \tabularnewline
		\centering{\bf{Moment of inertia}} & \multirow{2}{*}{\centering{1.23E-02}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{1.25E-02}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{1.97E-04}} \tabularnewline
		\centering{\bf{Spring stiffness}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{$\quad\; k_{l,\,eq}$}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{$\quad \;k_{t,\,eq}$}} \tabularnewline
		\centering{\bf{Damping ratio}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{0.00E+00}} & \multirow{2}{*}{\centering{0.00E+00}} \tabularnewline
		\centering{\bf{Loads}} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} & \centering{0.00E+00} \tabularnewline
		\centering{\bf{Mass}} & \centering{4.32E-01} & \centering{$\,$} & \centering{$\,$} & \centering{$\,$} & \centering{$\,$} & \centering{$\,$} \tabularnewline
		\centering{\bf{CCS}} & \centering{4.17E-02} & \centering{0.00E+00} & \centering{3.00E-01} & \centering{$\,$} & \centering{$\,$} & \centering{$\,$} \tabularnewline		
		\hline	
	\end{tabular}
	\caption{\label{table:csdvalues}Initialization file $csdvalues.dat$: Initial and boundary conditions, as well as system properties of the NACA0012 airfoil.}
\end{table}
\subsection{System stiffness}
\label{subsec:system_stiffness}
\par Since the experimental NACA0012-spring system (see Fig.\ \ref{fig:springs_NACA0012}) is characterized by the presence of four linear and two torsional springs, the total stiffness in each degree of freedom is calculated by the equivalent stiffness. 
\par Equations (\ref{eq:equivalent_linear_stiffness}) and (\ref{eq:equivalent_torsional_stiffness}) illustrate respectively the equivalent linear and torsional stiffnesses of the $x_2$ and $\varphi_3$ degrees of freedom, regarding parallel mounted springs. 
\begin{eqnarray}
\label{eq:equivalent_linear_stiffness}
k_{l\,2,\,eq}&=&k_{l\,2,1}+k_{l\,2,2}+k_{l\,2,3}+k_{l\,2,4}\\
\label{eq:equivalent_torsional_stiffness}
k_{t\,3,\,eq}&=&k_{t\,3,1}+k_{t\,3,2}
\end{eqnarray}

\subsection{Total mass}
\label{subsec:total_mass}
\par The mass of the airfoil is calculated according to Eq.\ (\ref{eq:mass_airfoil}). The chord and span-wise lengths, as well as the density of the experimental airfoil model are respectively $c=0.1\,m$,  $L_{3,\,N}=0.6\,m$ and $\rho_{N}=700\,kg{\cdot}m^{-3}$. $X_{N,\,2}$ describes the airfoil profile as a function of the chord length and the  $x_1$ coordinate (see Eq.\ (\ref{eq:NACA0012})). 
\begin{eqnarray}
m_{N}&=&2\;\rho_{N}\cdot L_{3,\,N}\int_{0}^{c}X_{N,\,1}\,dx_1
\label{eq:mass_airfoil}\\
m_{N}&=&0.3392\;\text{kg}\label{eq:mass_airfoil_value}
\end{eqnarray}
\par Since the experimental setup is characterized by the presence of two aluminum supports fixed on the airfoil (see Fig.\ \ref{fig:guiding_rod}) and these influence the dynamic equilibrium of the body, their masses ($m_\text{{supports}}=0.09299\,\text{kg}$) must be considered by the CSD solver. Therefore, the total mass $m_{tot}$ utilized in the $csdvalues.dat$ file is:
\begin{eqnarray}
\label{eq:total_mass}
m_{tot}&=&m_{N}+m_\text{{supports}}, \\
\label{eq:total_mass_value}
m_{tot}&=&0.43219\,\text{kg}.
\end{eqnarray}
\subsection{Center of mass}
\label{subsec:center_mass}
\par The undeformed body-fixed Cartesian coordinate system is located at the structure center of mass. Since the NACA0012 profile is symmetrical and the airfoil model has a span-wise length of $L_{3,\,N}=0.6\,m$, the $x_2$ and $x_3$ coordinates of the center of mass are respectively $x_{CM,\,2}=0\,m$ and $x_{CM,\,3}=0.3\,m$. The $x_1$ coordinate of the center of mass is calculated according to \mbox{Eq.\ (\ref{eq:mass_center_x})}, regarding that the density of the airfoil is constant.
\begin{eqnarray}
\label{eq:mass_center_x}
x_{CM,\,1}=\frac{\int_{0}^{c}x_1\,|X_{N,\,2}|\,dx_1}{\int_{0}^{c}|X_{N,\,2}|\,dx_1}=0.0417\,\text{m}
\end{eqnarray}
\par Due to the fact that the supports fixed on the airfoil are symmetric, their presence do not affect the location of the center of mass.

\subsection{Mass moment of inertia}
\label{subsec:moment_inertia}
\par In order to guarantee an uncoupled system, the origin of the body-fixed Cartesian coordinate system of the NACA0012 profile must be coincident with a Cartesian coordinate system constituted of only orthogonal to each other principal axes. These have the property of aligning the angular momentum $M_{ext,\,i}$ with the angular velocity $\dot{\varphi_i}$ and therefore are distinguished by the extinction of the products of inertia $J_{12}$, $J_{13}$ and $J_{23}$ \mbox{(see Hibbeler \cite{Hibbeler_2001}).} Since the airfoil is characterized by two axes that contain area symmetry ($x_1$ and $x_3$), when the body-fixed coordinate system is located at the body center of mass, these axes are considered principal axes (see Gere \cite{Gere_2004}). Moreover, any axis perpendicular to a principal axis is also a principal one, i$.$e$.$, $x_2$ is also a principal axis since it is orthogonal to $x_1$ and $x_3$. Hence, only the main diagonal of the mass moment of inertia tensor in relation to the center of mass of the NACA0012 airfoil remains, i$.$e$.$, the $J_{11}^{CM}$, $J_{22}^{CM}$ and $J_{33}^{CM}$ terms.
\par The mass moment of inertia is the quantity that indicates the object resistance to a rotational acceleration about a particular axis, i$.$e$.$, it indicates the distribution of the body mass in relation to a determined axis. The diagonal components of this tensor in relation to the global coordinate system ($J_{N,\,ii}^o$), which origin is located at the point O (see Fig.\ \ref{fig:points_O_CM}), are calculated according to Eqs.\ (\ref{eq:inertia_NACA_xx}) through (\ref{eq:inertia_NACA_zz}) for the NACA0012 airfoil. Although the profile function $X_{N,\,2}$ depends on the coordinate $x_1$, i$.$e$.$, $X_{N,\,2}(x_1)$, this is not repeatedly shown in the equations for the sake of brevity.
\begin{figure}[H]
	\centering
	\centering
	\includegraphics[scale=1,draft=\drafttype]{\FigPath/Masterarbeit/Global_local_coordinates.pdf}
	\caption{\label{fig:points_O_CM}O and CM: Origin of the global and local Cartesian coordinate systems, respectively.}
\end{figure}
\squeezeup
\begin{eqnarray}
\label{eq:inertia_NACA_xx}
\nonumber
J_{N,\,11}^o&=&\int_{V}\rho_N(x_2^2+x_3^2)\,dV=2\rho_N\int_{0}^{c}\int_{0}^{X_{N,\,2}}\int_{0}^{L_{3,\,N}}(x_2^2 + x_3^2)\;dx_3\,dx_2\,dx_1 \\
&=&\frac{2\,\rho_{N}}{3}\int_{0}^{c}\left(\left|X_{N,\,2}(x_1)\right|^3\,L_{3,\,N}+\left|X_{N,\,2}(x_1)\right|\,L_{3,\,N}^3\right)\,dx_1\\ \nonumber
\label{eq:inertia_NACA_yy}
J_{N,\,22}^o&=&\int_{V}\rho_N(x_1^2+x_3^2)\,dV=2\rho_N\int_{0}^{c}\int_{0}^{X_{N,\,2}}\int_{0}^{L_{3,\,N}}(x_1^2 + x_3^2)\;dx_3\,dx_2\,dx_1 \\
&=&2\,\rho_{N}\int_{0}^{c}\left(x_1^2\,\left|X_{N,\,2}(x_1)\right|\,L_{3,\,N}+\left|X_{N,\,2}(x_1)\right|\,\frac{L_{3,\,N}^3}{3}\right)\,dx_1\\ \nonumber
\label{eq:inertia_NACA_zz}
J_{N,\,33}^o&=&\int_{V}\rho_N(x_1^2+x_2^2)\,dV=2\rho_N\int_{0}^{c}\int_{0}^{X_{N,\,2}}\int_{0}^{L_{3,\,N}}(x_1^2 + x_2^2)\;dx_3\,dx_2\,dx_1 \\
&=&2\,\rho_{N}\,L_{3,\,N}\int_{0}^{c}\left(x_1^2\,|X_{N,\,2}(x_1)|+\frac{|X_{N,\,2}(x_1)|^3}{3}\right)\,dx_1
\end{eqnarray}
\par Since the undeformed body-fixed coordinate system is located at the airfoil center of mass CM, the mass moment of inertia tensor is then calculated in reference to this point. Therefore, the parallel axis theorem, i$.$e$.$, Huygens-Steiner theorem, is applied \mbox{(see Hibbeler \cite{Hibbeler_2001})}. This utilizes the perpendicular distances between the considered axis in the global and local coordinate systems, which origins are located respectively at points O and CM, in order to calculate the mass moment of inertia in relation to the airfoil center of mass, as stated in Eqs.\ (\ref{eq:inertia_NACA_CM_xx}) through (\ref{eq:inertia_NACA_CM_zz}):
\begin{eqnarray}
\label{eq:inertia_NACA_CM_xx}
J_{N,\,11}^{CM}=J_{N,\,11}^o-m_{N}\,x_{CM,\,3}^2=1.0200{\cdot}10^{-2}\;\text{kg}{\cdot}\text{m}^2,\\
\label{eq:inertia_NACA_CM_yy}
J_{N,\,22}^{CM}=J_{N,\,22}^o-m_{N}\,x_{CM,\,3}^2=1.1000{\cdot}10^{-2}\;\text{kg}{\cdot}\text{m}^2,\\
\label{eq:inertia_NACA_CM_zz}
J_{N,\,33}^{CM}=J_{N,\,33}^o-m_{N}\,x_{CM,\,1}^2=1.8687{\cdot}10^{-4}\;\text{kg}{\cdot}\text{m}^2.
\end{eqnarray}
\par The products of inertia $J_{N,\,ij}^{CM}$ at the center of mass are zero due to the fact that the coordinate axes are principal ones, as demonstrated in \mbox{Eqs.\ (\ref{eq:inertia_NACA_CM_xy}) through (\ref{eq:inertia_NACA_CM_yz})}:
\begin{eqnarray}
 \label{eq:inertia_NACA_CM_xy}\nonumber
 J_{N,\,12}^{CM}&=&\int_{A}x_1\,x_2\,dA=\int_{-x_{CM,\,1}}^{c-x_{CM,\,1}}\int_{-X_{N,\,2}}^{X_{N,\,2}}x_1\,x_2\;dx_2\,dx_1\\
 &=&\frac{1}{2}\int_{-x_{CM,\,1}}^{c-x_{CM,\,1}}x_1\left(X_{N,\,2}^2-X_{N,\,2}^2\right)dx_1=0\;\text{kg}{\cdot}\text{m}^2,
\end{eqnarray}
\begin{eqnarray}
% \label{eq:inertia_NACA_CM_xy}\nonumber
% &&\quad\quad\;\, J_{N,\,12}^{CM}\;\;=\;\;\int_{A}x_1\,x_2\,dA=\int_{-x_{CM,\,1}}^{c-x_{CM,\,1}}\int_{-X_{N,\,2}}^{X_{N,\,2}}x_1\,x_2\;dx_2\,dx_1\\
% &&\quad\quad\quad\quad\quad\;\;=\;\;\frac{1}{2}\int_{-x_{CM,\,1}}^{c-x_{CM,\,1}}x_1\left(X_{N,\,2}^2-X_{N,\,2}^2\right)dx_1=0\,kg{\cdot}m^2,\\ 
%\end{eqnarray}
%\begin{eqnarray}
\label{eq:inertia_NACA_CM_xz} \nonumber J_{N,\,13}^{CM}&=&\int_{A}x_1\,x_3\,dA=\rho_N\int_{V}x_1\,x_3\,dV=\rho_N\int_{-x_{CM,\,1}}^{c-x_{CM,\,1}}\int_{-X_{N,\,2}}^{X_{N,\,2}}\int_{-\frac{L_{3,\,N}}{2}}^{\frac{L_{3,\,N}}{2}}x_1\,x_3\;\,dx_3\,dx_2\,dx_1\\
&=&\frac{\rho_N}{2}\int_{-x_{CM,\,1}}^{c-x_{CM,\,1}}x_1\left(\frac{L_{3,\,N}^2}{4}-\frac{L_{3,\,N}^2}{4}\right)dx_1=0\;\text{kg}{\cdot}\text{m}^2,\\ \nonumber
\label{eq:inertia_NACA_CM_yz}
J_{N,\,23}^{CM}&=&\int_{A}x_2\,x_3\,dA=\rho_N\int_{V}x_2\,x_3\,dV=\rho_N\int_{-x_{CM,\,1}}^{c-x_{CM,\,1}}\int_{-X_{N,\,2}}^{X_{N,\,2}}\int_{-\frac{L_{3,\,N}}{2}}^{\frac{L_{3,\,N}}{2}}x_2\,x_3\;\,dx_3\,dx_2\,dx_1\\
&=&\frac{\rho_N}{2}\int_{-x_{CM,\,1}}^{c-x_{CM,\,1}}x_2\left(\frac{L_{3,\,N}^2}{4}-\frac{L_{3,\,N}^2}{4}\right)dx_1=0\;\text{kg}{\cdot}\text{m}^2.\\ \nonumber
\end{eqnarray}
\par The calculated airfoil mass moments of inertia are in great agreement with the ones calculated by a CAD software (see Fig.\ \ref{fig:airfoil_model_specifications}). Nevertheless, the presence of the supports fixed on the airfoil (see Fig.\ \ref{fig:guiding_rod}) also influence the rotational motion, therefore their mass moment of inertia are also considered. This results in slightly higher moments for the diagonal components while the products of inertia remain zero since the location of the principal axes are not altered, as presented in \mbox{Eq.\ (\ref{eq:inertia_total_CM})}:
\begin{equation}
\label{eq:inertia_total_CM}
J_{tot,\,ij}^{CM}=
\begin{bmatrix}
		1.22740{\cdot}10^{-2} & 0 & 0\\ 
		0 & 1.24656{\cdot}10^{-2} & 0\\
		0 & 0 & 1.97173{\cdot}10^{-4}
\end{bmatrix}
\;\text{kg}{\cdot}\text{m}^2.
\end{equation}

\subsection{Scaling of the fluid forces and moments}
\label{subsec:scaling_fluid_forces}
\par Since the simulated airfoil has a span-wise length of either $L_3=0.25\,c$ or $L_3=0.5\,c$ due to the utilization of a periodic boundary condition in this homogeneous direction and the system stiffness is not scaled in relation to the experimental setup, the fluid loads (forces and moments) must be geometrically scaled. This mathematical procedure assures the comparability of both numerical and experimental results and therefore enables a possible validation of the simulations. 
\begin{figure}[H]
	\centering
	\centering
	\includegraphics[scale=1.3,draft=\drafttype]{\FigPath/Masterarbeit/Lengths_airfoil_wind_tunnel.pdf}
	\caption{\label{fig:lengths_airfoil_wind_tunnel} Airfoil length submitted to the flow.}
\end{figure} 
\par Whereas the airfoil model has a span-wise length of $L_{3,\,N}=0.6\,m$, the test section of wind tunnel has a width of $L_{3,\,WT}=0.5\,m$ in order to guarantee the experimentation of an infinite airfoil (without the presence of wing tip turbulence), as illustrated in Fig.\ \ref{fig:lengths_airfoil_wind_tunnel}. The flow moves, then, only around the airfoil contained within the wind tunnel length $L_{3,\,WT}$. Therefore, as the CSD solver receives the fluid loads from FASTEST-3D, it primarily scales these values in relation to the length $L_{3,\,WT}$, as stated in \mbox{Eqs.\ (\ref{eq:scaling_forces}) and (\ref{scaling_moment})}:
\begin{eqnarray}
\label{eq:scaling_forces}F_{i,\,CSD}&=&F_i\cdot\frac{L_{3,\,WT}}{L_3},\\
\label{scaling_moment}
M_{i,\,CSD}&=&M_i\cdot\frac{L_{3,\,WT}}{L_3}.
\end{eqnarray}  
\par $F_{i,\,CSD}$ and $M_{i,\,CSD}$ represent the scaled forces and moments utilized by the CSD solver, while $F_i$ and $M_i$ represent the forces and moments calculated by the CFD solver. The scaling factor is composed of the length of the airfoil that is submitted to the flow $L_{3,\,WT}$ and the span-wise length of the airfoil in the CFD mesh $L_3$. 
\section{FSI setup}
\label{sec:FSI_setup}
\par The coupling algorithm explained in Section \ref{sec:coupling_fluid_structure} applies the FSI setup described in Table \ref{table:FSI_setup}: 
\begin{table}[!htbp]
	\centering
	\begin{tabular}{p{6.9cm} p{0.1cm} p{3.7cm}}
		\hline
		Under-relaxation of the fluid loads & & No \tabularnewline
		Under-relaxation of the displacements & & No \tabularnewline
		Coupling method & & Loose \tabularnewline
		Convergence criterion & & $\epsilon_{FSI,\,disp}<1{\cdot}10^{-6}$ \tabularnewline
		Estimation of displacements & & Linear extrapolation \tabularnewline
		\hline	
	\end{tabular}
	\caption{\label{table:FSI_setup}FSI setup.}
\end{table} 
\par The forces and displacements are not under-relaxed since the added mass effect is negligible (see Section \ref{subsec:added_mass_effect}) and convergence problems are not present. The negligibility of this effect also allows the utilization of a loose coupling method, which is proven to be accurate as well as less computational intensive, as thoroughly described in \mbox{Section \ref{subsec:investigation_coupling_algorithm}.} In order to save computational time, a prediction of the displacements at the next time step $n+1$ is utilized.



==> Makefile <==
#
#  Un exemple de Makefile pour fichiers LaTeX.
#
#  Exemples :
#	make,
#	make clean,
#	make all,
#	make xx.dvi,
#	make xx.ps,
#	...
#

TOP = report

LaTeX	= latex
BIBTEX	= bibtex

all:	$(TOP).pdf 
	pdflatex $(TOP).tex && bibtex $(TOP) && pdflatex $(TOP).tex && pdflatex $(TOP).tex && pdflatex $(TOP).tex

alllatex: $(TOP).pdf 
	latex $(TOP).tex && bibtex $(TOP) && latex $(TOP).tex && latex $(TOP).tex && dvips $(TOP).dvi && ps2pdf $(TOP).ps

clean:
	rm -rf $(TOP).dvi *.aux *.log $(TOP).toc \
	    $(TOP).lof $(TOP).lot $(TOP).ps $(TOP).bbl $(TOP).blg $(TOP).glo $(TOP).brf $(TOP).hd $(TOP).idx

new:
	make clean
	make all

newlatex:
	make clean
	make alllatex



==> chapter5.tex <==
\chapter{Results and discussion}
\label{chap:results}

\par Although various system configurations characterized by the same torsional\break stiffness of  \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$}, and by eleven different linear stiffnesses varying from \mbox{$k_{l\,2,\,eq}=40\,N{\cdot}m^{-1}$} to \mbox{$k_{l\,2,\,eq}=144\,N{\cdot}m^{-1}$} (see Appendix \ref{sec:flow_frequencies_re_meshing}) are simulated, the results achieved by all computations present the same pattern: After diverse initialization times, a limit-cycle oscillation (LCO) characterized by extremely small amplitudes, which are approximately equal for all simulations, is achieved. Since the test case with $k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$ requires the smallest computational time in order to achieve a fully developed state, this is thoroughly analyzed in the present work. 
\par The results are studied in a dimensionless manner when the flow is fully developed, regarding that the reference quantities are the airfoil chord $c$ and free stream velocity $u_{in,\,1}$.\break Firstly, the aerodynamic properties of the body are analyzed according to the time history of the drag and lift coefficients. Then, the airfoil displacements, as well as the aeroelastic properties are investigated. The latter is studied according to the frequencies generated by the flow and the oscillations. Finally, the instantaneous and time-averaged flow fields are investigated. A comparison with experimental data in order to validate the simulations is, however, not possible since the complete experimental setup is currently not available.

\section{Investigation of the aerodynamic properties}\markboth{CHAPTER 3.$\quad$RES. AND DISC.}{3.1$\quad$INV. OF THE AEROD. PROP.}
\label{sec:flow_forces}
\par The forces generated by the coupled problem are investigated according to the lift $C_L$ and drag $C_D$ coefficients. These non-dimensional numbers, which are proportional to the pressure and shear forces, are calculated according to Eqs.\ (\ref{eq:drag_coefficient}) and (\ref{eq:lift_coefficient}):
\begin{eqnarray}
\label{eq:lift_coefficient}
C_L&=&\frac{2\,F_L}{\rho_f\,S\,u_{in,\,1}^2},\\
\label{eq:drag_coefficient}
C_D&=&\frac{2\,F_D}{\rho_f\,S\,u_{in,\,1}^2}.
\end{eqnarray}
\par $F_D$, $F_L$, $u_{in,\,1}$, $\rho_f$ are respectively the drag and lift forces, the free stream velocity and the fluid density. The reference area $S$ is calculated according to Eq.\ (\ref{eq:reference_area}). $L_{3}$ and $c$ are the computational domain span-wise length and the airfoil chord length, i$.$e$.$, $L_{3}=0.025\,\text{m}$ and $c=0.1\,\text{m}$.
\begin{equation}
S=c\;L_{3} \label{eq:reference_area}
\end{equation}
\par The time history of the lift and drag coefficients are depicted in Fig.\ \ref{fig:drag_lift_history} for a dimensionless time interval of $1470\leq t^*\leq1500$. The initialization phase, which is present until about $t^*=600$, is not shown for the sake of brevity. In general, the period of the lift is higher than the period of the drag. However, the lift signal is also characterized by the presence of small periods, which might be caused by the Newmark method. 
\begin{figure}[H]
	\centering
	\subfigure[Drag coefficient.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/cd_kl_92.pdf} \label{fig:drag_history}}\hfill
	\subfigure[Lift coefficient.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/cl_kl_92.pdf}\label{fig:lift_history}}\hfill
	\caption{Time history of the drag and lift coefficients: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:drag_lift_history}
\end{figure}
\par The mean values and standard deviations of the lift and drag coefficients are summarized in Table \ref{table:mean_standard_aerodynamic_coefficients} considering a fully developed state. Although the standard deviation of the lift coefficient is about two orders of magnitude higher than the standard deviation of the drag coefficient, both aerodynamic coefficients weakly oscillate around a mean value. For the case of the lift coefficient, the mean value is approximately zero, which indicates that the symmetric NACA0012 airfoil is at an incidence of $\alpha=0^\circ$. Moreover, the lift and drag coefficients for the coupled problem are about the same of the ones calculated for the case characterized by a fixed airfoil (see Section \ref{sec:study_span_wise_length})
\begin{table}[H]
	\centering
	\begin{tabular}{p{2.4cm} p{4cm} p{0.2cm} p{2.4cm} p{4cm}}
		\hline
		\multicolumn{2}{c}{\textbf{Drag coefficient}} & & \multicolumn{2}{c}{\textbf{Lift coefficient}} \tabularnewline \cline{1-2} \cline{4-5}
		\centering{\textbf{Mean value}} & \centering{\textbf{Standard deviation}} & & \centering{\textbf{Mean value}} & \centering{\textbf{Standard deviation}} \tabularnewline
		\hline
		\centering{$2.48{\cdot}10^{-2}$} & \centering{$8.02{\cdot}10^{-4}$} & & \centering{$4.95{\cdot}10^{-4}$} & \centering{$1.79{\cdot}10^{-2}$} \tabularnewline
		\hline			
	\end{tabular}
	\caption{\label{table:mean_standard_aerodynamic_coefficients}Mean values and standard deviations of the aerodynamic coefficients: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,\text{N}{\cdot}\text{m}{\cdot}\text{rad}^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,\text{N}{\cdot}\text{m}^{-1}$}.}
\end{table}
\section{Investigation of the airfoil displacements}\markboth{CHAPTER 3.$\quad$RES. AND DISC.}{3.2$\quad$INV. OF THE AIRFOIL. DISP.}
\label{sec:airfoil_response}
\par The fluid forces and moments act on the airfoil and generate displacements in relation to the plunge and pitch degrees of freedom. These displacements are illustrated in \mbox{Fig.\ \ref{fig:pitch_plunge_history}} in relation to the dimensionless time $t^*$, regarding that the high frequencies are present in the pitch motion. After the transitional phase, which is present until $t^*\approx600$, a limit-cycle oscillation is generated, which is characterized by weak oscillations around a mean value. This value, as well as the standard deviation of both displacements are described in Table \ref{table:mean_standard_displacements}.
\begin{figure}[H]
	\centering
	\subfigure[Translational displacement $X_2$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/plunge_kl_92.pdf} \label{fig:plunge_history}}\hfill
	\subfigure[Translational displacement $X_2$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/plunge_zoom_kl_92.pdf} \label{fig:plunge_zoom_history}}\hfill
	\subfigure[Rotational displacement $\varphi_3$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pitch_kl_92.pdf}\label{fig:pitch_history}}\hfill
	\subfigure[Rotational displacement $\varphi_3$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pitch_zoom_kl_92.pdf}\label{fig:pitch_zoom_history}}\hfill
	\caption{Time history of the translational and rotational displacements: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:pitch_plunge_history}
\end{figure}
\begin{table}[H]
	\centering
	\begin{tabular}{p{2.4cm} p{4cm} p{0.2cm} p{2.4cm} p{4cm}}
		\hline
		\multicolumn{2}{c}{\textbf{Translational displacement $X_2$ (m)}} & & \multicolumn{2}{c}{\textbf{Rotational displacement $\varphi_3$ ($^\circ$)}} \tabularnewline \cline{1-2} \cline{4-5}
		\centering{\textbf{Mean value}} & \centering{\textbf{Standard deviation}} & & \centering{\textbf{Mean value}} & \centering{\textbf{Standard deviation}} \tabularnewline
		\hline
		\centering{$3.44{\cdot}10^{-6}$} & \centering{$3.27{\cdot}10^{-5}$} & & \centering{$2.70{\cdot}10^{-6}$} & \centering{$8.62{\cdot}10^{-5}$} \tabularnewline
		\hline			
	\end{tabular}
	\caption{\label{table:mean_standard_displacements}Mean values and standard deviations of the airfoil displacements: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
\end{table}
\par The limit-cycle amplitudes of the pitch and plunge motions are extremely small, which is expected for the current test case. This phenomenon arises for fluid structure interactions of the NACA0012 airfoil at low to moderate chord Reynolds numbers \mbox{($15{,}000 \leq Re\leq 500{,}000$)} either when no angular and plunging velocities are initially available and the airfoil is at an incidence of \mbox{$\alpha=0^\circ$} \mbox{(see Lapointe and Dumas \cite{Lapointe_2012})}, or when the linear stiffness is small, i$.$e$.$, roughly $k_{l\,2,\,eq}\leq300\,N{\cdot}m^{-1}$ (see Poirel and Mendes \cite{Poirel_2012}). 
\par An increase of the linear stiffness up to $k_{l\,2,\,eq}=144\,N{\cdot}m^{-1}$, which is the maximal linear stiffness available for the experiments (see Appendix \ref{appendix_experimental_setup}), leads to an increase in the amplitudes of the pitch and plunge motions. However, the limit-cycle oscillation is still characterized by extremely small amplitudes. 
\begin{figure}[H]
	\centering
	\subfigure[Translational displacement $X_2$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/plunge_comp_kl.pdf} \label{fig:plunge_comp_kl_history}}\hfill
	\subfigure[Translational displacement $X_2$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pitch_comp_kl.pdf} \label{fig:pitch_comp_kl_history}}\hfill
	\caption{Time history of the translational and rotational displacements: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:plunge_pitch_comp_kl}
\end{figure}
\begin{figure}[H]
	\centering
	\centering
	\includegraphics[width=0.49\textwidth,draft=\drafttype]{\FigPath/Masterarbeit/pitch_comp_1DOF_2DOF.pdf}
	\caption{\label{fig:pitch_comp_history}Time history of the rotational displacements regarding a torsional stiffness of \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$}: Cases with and without plunge degree of freedom.}
\end{figure}
\par Moreover, Lapointe and Dumas \cite{Lapointe_2012} stated that if a fluid-structure interaction is characterized by LCO with small amplitudes, then these amplitudes are similar to the ones achieved with cases characterized by only the pitch degree of freedom. Therefore, Fig.\ \ref{fig:pitch_comp_history} illustrates a comparison of the rotational displacements achieved by the current test case (\mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}) and by the computation with only the pitch degree of freedom (\mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$}). As expected, the achieved pitching amplitudes are very similar in both cases.


\section{Investigation of the frequencies}
\label{sec:frequencies}

\par The aerodynamic forces, as well as the displacements are characterized by an oscillatory behavior. Therefore, Fourier transforms are applied in order to analyze the frequency domain of these variables. In order to acquire accurate results the available data is firstly post-processed in order to obtain oscillations composed of only complete periods. The Fourier transform is then applied, considering that rectangular, triangular, Hann and Hamming window functions are investigated and deliver the exact same result.

\subsection{Flow frequencies}
\label{subsec:flow_frequencies}

\par The frequencies generated by the drag and lift forces are analyzed aiming primarily at the identification of the vortex shedding frequency $f_v$. This is required in order to calculate the Strouhal number $St$, which is a dimensionless number that characterizes unsteady flow mechanisms, i$.$e$.$, it describes the oscillatory phenomenon available in a flow. In the current work, this dimensionless number is a function of the vortex shedding frequency $f_v$, the airfoil chord $c=0.1\,m$ and the free stream velocity $u_{1,\,in}=4.47\,m{\cdot}s^{-1}$, as described in Eq.\ (\ref{eq:strouhal_number}):
\begin{equation}
\label{eq:strouhal_number}
St=\frac{f_{v}\,c}{u_{1,\,in}}.
\end{equation}

\par The frequency domain of the drag and lift forces is depicted in Fig.\ \ref{fig:frequency_forces}, regarding that an overall view of this domain, as well as a view focused on the low frequencies are available.
\begin{figure}[H]
	\centering
	\subfigure[Overall frequency domain: Drag.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/frequencies_drag_kl_92.pdf} \label{fig:frequency_drag}}\hfill
	\subfigure[Focus on the low frequencies: Drag.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/frequencies_drag_zoom_kl_92.pdf} \label{fig:frequency_zoom_drag}}\hfill
\end{figure}
\begin{figure}[H]
	\subfigure[Overall frequency domain: Lift.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/frequencies_lift_kl_92.pdf} \label{fig:frequency_lift}}\hfill
	\subfigure[Focus on the low frequencies: Lift.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/frequencies_lift_zoom_kl_92.pdf} \label{fig:frequency_zoom_lift}}\hfill
	\caption{Frequency domain of the drag and lift forces: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:frequency_forces}
\end{figure}
\par Both frequency domains are characterized by the presence of many strong peaks. In the case of high frequencies, the drag frequency domain is characterized by a frequency of $f_D^h=58.61\,Hz$, which super-harmonics at $2f_D^h$, $3f_D^h$, $4f_D^h$, $5f_D^h$ and $6f_D^h$ are present. The high frequencies generated by the lift are characterized mainly by the frequency $f_L^h=55.6\,Hz$. Although no exact super-harmonic of this frequency is present, many peaks at frequencies near the super-harmonic ones are present. This shift could be a result of a interaction with the Newmark method, since this numerically generates high frequencies. 
\par The high frequencies of the drag and lift forces are not related to the vortex shedding. On the other hand, these are possibly related to some instability generated by the geometry of the structure or by the structure itself, since its natural frequencies are high, i$.$e$.$, respectively $w_{n,\,2}=18.25\,Hz$ and $w_{n,\,3}=44.08\,Hz$ for the plunge and pitch degrees of freedom. The exactly nature of these frequencies is, however, not thoroughly investigated in the current work.
\par The low frequency domain is characterized by frequencies related uniquely to the flow, which are illustrated in Table \ref{table:flow_frequencies} together with the dimensionless Strouhal number. Both domains present the same pattern: a strong peak at $f_L$ and $f_D$ is available and these are followed by the super-harmonics, which points out the strength of the flow nonlinearities. The drag frequency is approximately twice the value of the lift frequency, indicating the presence of a von  K\'arm\'an vortex street \mbox{(see Manhart \cite{Manhart_1998})}. This instability is characterized by a periodic detachment of pairs of alternating vortices and is thoroughly explored in \mbox{Section \ref{sec:instationary_flow_field}}. Due to the presence of this instability, the vortex shedding frequency is equal to the lift frequency. Therefore, the Strouhal number in relation to the chord length is $St=0.068$. This dimensionless number is qualitatively compared to the one achieved by Poirel et al.\ \cite{Poirel_2008}, who experimentally studied self-sustained aeroelastic oscillations of a NACA0012 airfoil at a Reynolds number range of $4.5{\cdot}10^4\leq Re\leq1.3{\cdot}10^5$ and achieved a Strouhal number range of $0.05\leq St\leq0.07$. Since the decrease of the Reynolds number leads to an increase of the vortex shedding period and therefore an increase of the vortex shedding frequency, the highest Strouhal numbers are achieved for the lowest Reynolds numbers. Hence, the results achieved in the present work are in agreement with the experimental results of Poirel et al$.$. 

\begin{table}[H]
	\centering
	\begin{tabular}{p{3.5cm} p{3.4cm} p{4cm} p{3cm}}
	\hline
	\centering{\textbf{Drag frequency $f_D$ (Hz)}} & \centering{\textbf{Lift frequency $f_L$ (Hz)}} & \centering{\textbf{Vortex shedding frequency $f_v$ (Hz)}} & \centering{\textbf{Strouhal number $St$}} \tabularnewline \hline
	\centering{3.03} & \centering{6.05} & \centering{3.03} & \centering{0.068} \tabularnewline
	\hline
	\end{tabular}
	\caption{\label{table:flow_frequencies}Flow frequencies and Strouhal number: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
\end{table}

\subsection{Structural frequencies}
\label{subsec:structural_frequencies}
\par The frequencies generated by the translational and rotational displacements are thoroughly investigated according to Fig.\ \ref{fig:frequency_displacements} and Table \ref{table:structural_frequencies}. Although high frequencies are not illustrated, a frequency of $f_{\varphi_3}^h=55.54\,Hz$ is generated by the pitch oscillation. This is similar to the high frequency generated by the lift forces $f_L^h=55.6\,Hz$ \mbox{(see Section \ref{subsec:flow_frequencies})} and might be related to the structure itself.
\begin{figure}[H]
	\centering
	%\subfigure[Translational displacement $X_2$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/frequencies_X2_kl_92.pdf} \label{fig:plunge_comps_kl_history}}\hfill
	\subfigure[Translational displacement $X_2$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/frequencies_X2_zoom_kl_92.pdf} \label{fig:pitch_comp_kls_history}}\hfill
	%\subfigure[Rotational displacement $\varphi_3$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/frequencies_phi3_kl_92.pdf} \label{fig:plunge_comp_ksl_history}}\hfill
	\subfigure[Rotational displacement $\varphi_3$.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/frequencies_phi3_zoom_kl_92.pdf} \label{fig:pitch_comp_kl_hsistory}}\hfill
	\caption{Frequency domain of the drag and lift forces: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:frequency_displacements}
\end{figure}
\begin{table}[H]
	\centering
	\begin{tabular}{p{6cm} p{6cm}}
		\hline
		\centering{\textbf{Plunge frequency $f_{X_{2}}$ (Hz)}} & \centering{\textbf{Pitch frequency $f_{\varphi_{3}}$ (Hz)}}  \tabularnewline \hline
		\centering{3.03} & \centering{3.03} \tabularnewline
		\hline
	\end{tabular}
	\caption{\label{table:structural_frequencies}Plunge and pitch frequencies: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
\end{table}
\par The frequency domain of the displacements is characterized by the generation of mainly low frequencies, considering that super-harmonics are available in the pitch movement. Moreover, both domains present the same frequency, which is also equal to the vortex shedding frequency. Therefore, the small LCO is caused mainly by the vortex shedding present on the airfoil trailing edge.  

\section{Investigation of the instantaneous flow field}\markboth{CHAPTER 3.$\quad$RES. AND DISC.}{3.4$\quad$INV. OF THE INST. FLOW FIELD}
\label{sec:instationary_flow_field}
\par The instantaneous flow field is studied according to the velocity, pressure, pressure fluctuation, as well as normalized span-wise vorticity and vorticity magnitude. Since the achieved LCO is characterized by extremely small displacements and the vortex shedding frequency is equal to the frequency of the structural displacement (see Section \ref{sec:frequencies}), this investigation aims specially at the study of the vortex shedding.
\par The temporal progress of the fully developed instantaneous flow field for a complete cycle of the structural displacement is thoroughly analyzed through figures at $t$, \mbox{$t+0.25\,T_v$}, $t+0.5\,T_v$ and $t+0.75\,T_v$. The former illustrates the beginning of the oscillation, considering a sinusoidal wave. The second depicts the crest of the wave and is followed by an image at the oscillation mean value. Finally, the wave trough is illustrated. $t$ represents an arbitrary time and $T_v$ is the vortex shedding period, i$.$e$.$, $T_v\approx0.33$.
\par The dimensionless instantaneous velocity in the stream-wise direction is illustrated in \mbox{Fig.\ (\ref{fig:velocity_development})}. A boundary layer detachment is present at $x^*=0.8\,m$ (see Section \ref{sec:time_avg_flow_field}). This is responsible for the shed of vortices that travel downstream and interact with the structure, leading to extremely small structure oscillations, which cannot be distinguished in the figures.   
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vel_1.pdf} \label{fig:velocity_1}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vel_2.pdf}\label{fig:velocity_2}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vel_3.pdf}\label{fig:velocity_3}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vel_4.pdf}\label{fig:velocity_4}}\hfill
	\caption{Temporal development of the dimensionless stream-wise velocity field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:velocity_development}
\end{figure}
\par The unsteady pressure field is depicted in Fig.\ \ref{fig:pressure_development}. This is approximately symmetric in the first half of the profile due to the symmetry of the airfoil and the applied Reynolds number, which is characterized by a laminar flow until the boundary layer is detached (see Section \ref{sec:time_avg_flow_field}). After the detachment point, the flow is turbulent and characterized by the formation of vortices. Moreover, the unbalanced distribution of the pressure near the airfoil trailing edge lead to the minimal oscillation of the airfoil.
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_1.pdf} \label{fig:pressure_1}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_2.pdf}\label{fig:pressure_2}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_3.pdf}\label{fig:pressure_3}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_4.pdf}\label{fig:pressure_4}}\hfill
	\caption{Temporal development of the dynamic pressure field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:pressure_development}
\end{figure}
\par Since the swirling direction of the vortices, as well as the vortex cores cannot be identified solely with the unsteady velocity and pressure fields, the pressure fluctuation $p'$, the span-wise vorticity $\omega_{f,\,3}$ and the vorticity magnitude $\omega_f$ are also displayed, considering that these values are calculated according to Eqs.\ (\ref{eq:pressure_fluctuation}) through (\ref{eq:vorticity_mag}). ${<}p{>}$ represents the time-averaged pressure.
\begin{eqnarray}
\label{eq:pressure_fluctuation}
&&\quad\quad\quad\quad\quad\quad p'\quad=\quad p\,\,-\,{<}p{>},\\
\label{eq:vorticity_z}
&&\quad\quad\quad\quad\quad \omega_{f,\,3}\quad=\quad\frac{\partial u_2}{\partial x_1}- \frac{\partial u_1}{\partial x_2},\\ \label{eq:vorticity_mag}
\omega_{f}&=&\sqrt{\left(\frac{\partial u_3}{\partial x_2}- \frac{\partial u_2}{\partial x_3}\right)^2+\left(\frac{\partial u_1}{\partial x_3}- \frac{\partial u_3}{\partial x_1}\right)^2+\left(\frac{\partial u_2}{\partial x_1}- \frac{\partial u_1}{\partial x_2}\right)^2}.
\end{eqnarray} 
\par The position of vortex cores, as well as stagnation points can be investigated according to the pressure fluctuation, considering that regions with negative pressure fluctuations correspond to vortex cores whereas regions of positive pressure fluctuation indicate the position of stagnation points in the turbulent flow field \cite{Manhart_1998}. Figure \ref{fig:pressure_fluctuation_delevopment} shows the pressure fluctuation field, which is characterized by the presence of vortex cores in the wake.
\par In order to precisely analyze the art of vortex shedding present near the airfoil trailing edge, the vorticity in the span-wise direction is studied, as illustrated in Fig.\ \ref{fig:vorticity_z_development}. A negative vorticity indicates that the vortex rolls in the clockwise direction, while a positive vorticity evinces a counter-clockwise rotation \cite{Streher_2017}. Therefore, a K\'arm\'an vortex street, i$.$e$.$, a repeating pattern of alternating swirling vortices, can be identified. The vortices formed on the suction side rotate in clockwise direction, while the vortices shed on the pressure side rotate in the counter-clockwise direction.
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_fluc_1.pdf} \label{fig:pressure_fluc_1}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_fluc_2.pdf}\label{fig:pressure_fluc_2}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_fluc_3.pdf}\label{fig:pressure_fluc_3}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_fluc_4.pdf}\label{fig:pressure_fluc_4}}\hfill
	\caption{Temporal development of the pressure fluctuation field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:pressure_fluctuation_delevopment}
\end{figure}
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_z_1.pdf} \label{fig:vorticity_z_1}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_z_2.pdf}\label{fig:vorticity_z_2}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_z_3.pdf}\label{fig:vorticity_z_3}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_z_4.pdf}\label{fig:vorticity_z_4}}\hfill
	\caption{Temporal development of the normalized span-wise vorticity field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:vorticity_z_development}
\end{figure}
\par Finally, the vorticity magnitude normalized in relation to the maximal value is depicted in Fig.\  \ref{fig:vorticity_mag_development}. This clearly illustrates the formation of the vortices. Moreover, the boundary layer detachment near the airfoil can also be identified, since this is characterized by small magnitudes of the vorticity.
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_mag_1.pdf} \label{fig:vorticity_mag_1}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_mag_2.pdf}\label{fig:vorticity_mag_2}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_mag_3.pdf}\label{fig:vorticity_mag_3}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_mag_4.pdf}\label{fig:vorticity_mag_4}}\hfill
	\caption{Temporal development of the normalized vorticity magnitude field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:vorticity_mag_development}
\end{figure}
\markboth{CHAPTER 3.$\quad$RES. AND DISC.}{3.4$\quad$INV. OF THE TIME-AVG. FLOW FIELD}
\section{Investigation of the time-averaged flow field}\markboth{CHAPTER 3.$\quad$RES. AND DISC.}{3.4$\quad$INV. OF THE TIME-AVG. FLOW FIELD}
\label{sec:time_avg_flow_field}

\par Although the current work describes the fluid-structure interaction of the NACA0012 profile, the amplitudes of the limit-cycle oscillations are so small that the time-averaged flow field can be investigated. The unsteady flow field is, then, averaged for a time period equivalent of about 30 vortex shedding cycles aiming at the investigation of complex viscous phenomena. % that are characteristics of the highly nonlinear flow around the NACA0012 at low-to-moderade chord Reynolds numbers, i$.$e$.$, \mbox{$15{,}000\leq Re\leq 500{,}000$} (see Jones et al.\ \cite{Jones_2008} and Visbal et al.\ \cite{Visbal_2009}).
%\par The averaged streamlines are analyzed according to Fig.\ \ref{fig:streamlines_avg}:
\begin{figure}[H]
	\centering
	\subfigure[Overall view.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/streamlines_avg_kl_92.pdf} \label{fig:streamlines_overall}}\hfill
	\subfigure[Focus on the trailing edge.]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/streamlines_avg_kl_92_zoom.pdf}\label{fig:streamlines_zoom}}\hfill
	\caption{Time-averaged streamlines: Case with $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:streamlines_avg}
\end{figure}
\par According to Fig.\ \ref{fig:streamlines_avg}, a detachment of the boundary layer is present near the trailing edge on the suction and pressure sides of the airfoil, i$.$e$.$, at $x_{DP}^*=0.8$. This is not reattached further downstream and is responsible for the formation of a von K\'ar\'an vortex street (see Section \ref{sec:instationary_flow_field}).
\par The distribution of the Reynolds stresses around the NACA0012 airfoil confirms that the flow at $Re=30{,}000$ is in a sub-critical regime, i$.$e$.$, it is laminar. The transition to a turbulent regime occurs after the detachment point, which leads to a turbulent wake. This is illustrated in Fig.\ \ref{fig:reynolds_stresses_avg} for the $\tau_{11}^{turb^{*}}$ $\tau_{12}^{turb^{*}}$ and $\tau_{22}^{turb^{*}}$ Reynolds stresses components. 
\begin{figure}[H]
	\centering
	\subfigure[$\tau_{11}^{turb^{*}}$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/uu_kl_92.pdf} \label{fig:uu}}\hfill
	\subfigure[$\tau_{12}^{turb^{*}}$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/uv_kl_92.pdf}\label{fig:uv}}\hfill
	\subfigure[$\tau_{22}^{turb^{*}}$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vv_kl_92.pdf}\label{fig:vv}}\hfill
	\caption{Time-averaged Reynolds stresses: Test case at $Re=30{,}000$ and with \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:reynolds_stresses_avg}
\end{figure}
\par Poirel et al.\ \cite{Poirel_2011} observed that a turbulent regime inhibit the existence of limit-cycle oscillations. Therefore, the existing laminar flow field influence the generation of the small LCO. Moreover, Poirel and Yuan \cite{Poirel_2010} studied self-sustained pitch oscillations of a NACA0012 airfoil at transitional Reynolds numbers ($50{,}000\leq Re\leq130{,}000$) and suggested that laminar separation leading to the formation of a laminar separation bubble plays a key role in the oscillations. Although the current work computes the fluid domain at a Reynolds number of $Re=30{,}000$ and the airfoil has plunge and pitch degrees of freedom, the presence of only a laminar separation at the airfoil trailing edge, i$.$e$.$, the absence of a laminar separation bubble, might be related to the small LCO achieved by the fluid-structure interaction of the NACA0012 airfoil.




\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par
\par


\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_1_lift.pdf} \label{fig:frequsencies_hsigh_high_kl}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_2_lift.pdf}\label{fig:oisfrsequencies_shigh_kl}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_3_lift.pdf}\label{fig:oifsrsequencies_hsigh_kl}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_4_lift.pdf}\label{fig:oifrssequencies_hisgh_kl}}\hfill
	\caption{Temporal development of the dynamic pressure field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:frequencies_all_kssl}
\end{figure}
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_fluc_1_lift.pdf} \label{fig:fsrequsencies_high_high_kl}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_fluc_2_lift.pdf}\label{fig:oissfrsequencies_high_kl}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_fluc_3_lift.pdf}\label{fig:oifssrsequencies_high_kl}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/pres_fluc_4_lift.pdf}\label{fig:oifrsssequencies_high_kl}}\hfill
	\caption{Temporal development of the pressure fluctuation field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:frequencies_all_ksssl}
\end{figure}
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vel_1_lift.pdf} \label{fig:velocity_1}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vel_2_lift.pdf}\label{fig:velocity_2}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vel_3_lift.pdf}\label{fig:velocity_3}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vel_4_lift.pdf}\label{fig:velocity_4}}\hfill
	\caption{Temporal development of the dimensionless stream-wise velocity field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:velocity_development}
\end{figure}
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_z_1_lift.pdf} \label{fig:fsrequsencfies_high_high_kl}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_z_2_lift.pdf}\label{fig:oissfrsequenfcies_high_kl}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_z_3_lift.pdf}\label{fig:oifssrsequencfies_high_kl}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_z_4_lift.pdf}\label{fig:oifrsssequencifes_high_kl}}\hfill
	\caption{Temporal development of the normalized span-wise vorticity field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:frequencies_all_ksssfl}
\end{figure}
\begin{figure}[H]
	\centering
	\subfigure[$t$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_mag_1_lift.pdf} \label{fwig:fsrequsencies_high_high_kl}}\hfill
	\subfigure[$t+0.25\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_mag_2_lift.pdf}\label{figw:oissfrsequencies_high_kl}}\hfill
	\subfigure[$t+0.5\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_mag_3_lift.pdf}\label{fig:woifssrsequencies_high_kl}}\hfill
	\subfigure[$t+0.75\,T_v$]{\includegraphics[width=0.49\textwidth]{\FigPath/Masterarbeit/vorticity_mag_4_lift.pdf}\label{fig:owifrsssequencies_high_kl}}\hfill
	\caption{Temporal development of the normalized vorticity magnitude field: Test case characterized by $Re=30{,}000$, \mbox{$k_{t\,3,\,eq}=0.3832\,N{\cdot}m{\cdot}rad^{-1}$} and \mbox{$k_{l\,2,\,eq}=92\,N{\cdot}m^{-1}$}.}
	\label{fig:frequencies_all_ksswsl}
\end{figure}


==> corporate/TV.tex <==
%-----------------------------------------------------------------------------------------------------
% Allgemeine Titeldaten
%-----------------------------------------------------------------------------------------------------

\addresshead{Helmut-Schmidt-Universität}
\address{Universität der Bundeswehr Hamburg\\Postfach 70 08 22\\22008 Hamburg}

\faculty{Maschinenbau}
\department{Professur für Mechatronik}
\professor{Univ.-Prof. Dr.-Ing.  Franz Joos\\Betreuer: M.Sc.Eng. Dipl.-Ing Tim Nowakowski}

\endinput


==> corporate/mechatronik.tex <==
%-----------------------------------------------------------------------------------------------------
% Allgemeine Titeldaten
%-----------------------------------------------------------------------------------------------------

\addresshead{Helmut-Schmidt-Universität}
\address{Universität der Bundeswehr Hamburg\\Postfach 70 08 22\\22008 Hamburg}

\faculty{Maschinenbau}
\department{Professur für Mechatronik}
\professor{Univ.-Prof. Dr.-Ing.  Delf Sachau\\Dr.-Ing. Thomas Kletschkowski}

\endinput


==> corporate/messtechnik.tex <==
%-----------------------------------------------------------------------------------------------------
% Allgemeine Titeldaten
%-----------------------------------------------------------------------------------------------------

\addresshead{Helmut-Schmidt-Universität}
\address{Universität der Bundeswehr Hamburg\\Postfach 70 08 22\\22008 Hamburg}

\faculty{Maschinenbau}
\department{Professur für Mess- und Informationstechnik}
\professor{ Univ.- Prof. Dr.- Ing. habil.  Hendrik  Rothe}

\endinput


==> first_page.tex <==
\maketitle

	

